Harmonic Chain Barcode and Stability

The persistence barcode is a topological descriptor of data that plays a fundamental role in topological data analysis. Given a filtration of the space of data, a persistence barcode tracks the evolution of its homological features. In this paper, we introduce a novel type of barcode, referred to as the canonical barcode of harmonic chains, or harmonic chain barcode for short, which tracks the evolution of harmonic chains. As our main result, we show that the harmonic chain barcode is stable and it captures both geometric and topological information of data. Moreover, given a filtration of a simplicial complex of size $n$ with $m$ time steps, we can compute its harmonic chain barcode in $O(m^2n^{\omega} + mn^3)$ time, where $n^\omega$ is the matrix multiplication time. Consequently, a harmonic chain barcode can be utilized in applications in which a persistence barcode is applicable, such as feature vectorization and machine learning. Our work provides strong evidence in a growing list of literature that geometric (not just topological) information can be recovered from a persistence filtration.

==> sec-background.tex <==
\section{Background}
\label{sec:background}

In this section, we review the notion of harmonic chains and persistent homology; see~\cref{sec:homology} for a review of standard notions of homology and cohomology with real coefficients. 
Let $K$ be a simplicial complex and $p$ the homology dimension. 
$C_p(K)$, $Z_p(K)$, and $H_p(K)$ denote the $p$-th chain group, cycle group, and homology group of $K$.
$C^p(K)$, $Z^p(K)$, and $H^p(K)$ denote the $p$-th cochain group, cocycle group, and cohomology group of $K$.
$\partial$ and $\delta$ denote boudary and coboundary operators, respectively. 

\subsection{Harmonic Cycles} 
Based on the standard notions of homology and cohomology (see~\cref{sec:homology}), we identify chains and cochains via duality and identify both with a Euclidean vector-space $\Rspace^{n_p}$, where $n_p$ is the number of $p$-simplices.  
Therefore, we can talk about the coboundary of the cycles $Z_p(K)$. The \textit{harmonic $p$-cycles}, denoted $\har_p(K)$ is the group of those cycles which are also cocylces. Considered as subspaces of $\Rspace^{n_p}$, we have $\har_p(K) = Z^p(K) \cap Z_p(K)$.

\begin{lemma}[\cite{eckmann1944harmonische}]
    $\har_p(K)$ is isomorphic to $H_p(K)$. In other words, each homology class has a unique harmonic cycle in it.
\end{lemma}

Harmonic cycles enjoy certain geometric properties. As an example we mention the following \Cref{prop:uniqueness}. For a proof see~\cite[Proposition 3]{deSilvaVejedomo}. In other words, the harmonic chain is the chain with the least squared-norm in a cohomology class.

\begin{proposition}
\label{prop:uniqueness}
    Let $\alpha \in C^p(K)$ be a cochain. There is a unique solution $\bar{\alpha}$ to the least-squares minimization problem $$ \text{argmin}_{\bar{\alpha}} \{ || \bar{\alpha}||^2 \; | \; \exists \gamma \in C^{p-1}(K);  \alpha = \bar{\alpha}+\delta \gamma \}.$$ Moreover, $\bar{\alpha}$ is characterised by the relation $\partial {\bar{\alpha}}=0$.
\end{proposition}




\subsection{Persistent Homology}

Persistent homology tracks the changes in homology over time (or any other  parametrization).  
We start with a filtration $F$ of a simplicial complex $K$. A filtration assigns to each $r\in \Rspace$ a subcomplex $K_r \subset K$, in such a way that, if $r \leq s$, then $K_r \subseteq K_s$. 
Since $K$ is finite, there is a finite set of values $t_1, \ldots, t_m \in \Rspace$ where the subcomplex $F_{t_i}$ changes. Setting $K_i = K_{t_i}$, $K_0 = \emptyset$, $K_i \hookrightarrow K_{i+1}$ the inclusions, the filtration $F$ can be written as
\begin{equation}
\label{eq:fcomplex}
    \emptyset = K_0 \hookrightarrow K_1 \hookrightarrow \cdots \hookrightarrow K_{m-1} \hookrightarrow K_m=K.
\end{equation}

Applying homology functor to Eqn.~\eqref{eq:fcomplex}, we obtain a sequence of homology groups and connecting homomorphisms (linear maps), forming a \textit{persistence module}:
\begin{equation}\label{eq:fhomology}
 H_p(K_0) \xrightarrow{f_p^{t_0,t_1}} H_p(K_1) \xrightarrow{f_p^{t_1,t_2}}   \cdots \xrightarrow{f_{p}^{t_{m-2},t_{m-1}}} H_p(K_{m-1}) \xrightarrow{f_{p}^{t_{m-1},t_m}} H_p(K_m).   
\end{equation} 
In general, a persistence module $M$ at dimension $p$ is defined as assigning to each $r\in \Rspace$ a vector space $M_r$, and for each pair $s<t$, a homomorphism $f_p^{s,t}: M_s \xrightarrow{} M_t$. For all $s<t<u$, the homomorphism are required to satisfy linearity, that is, $f_p^{t,u} \circ f_p^{s,t}= f_p^{s,u}$. 

A cycle $z \in Z_p(K)$ appears for the first time at some index $b \in \{t_0,\ldots,t_m\}$, where it creates a new homology class in $K_b$ not previously existing. We say that the homology class is \textit{born} at time $b$. 
The homology class then lives for a while until it \textit{dies} entering $K_d$, when is not in the image of the map induced on homology by the inclusion $K_b \subset K_d$. 
For $s\leq t$, let $f^{s,t}_p: H_p(K_s) \rightarrow H_p(K_t)$ denote the map induced on the $p$-dimensional homology by the inclusion $K_s \subset K_t$. 
The image of this homomorphisms, $f^{s,t}_p(H_p(K_s)) \subset H_p(K_t)$, is called the $p$-dimensional \textit{$(s,t)$-persistent homology group}, denoted $H_p^{s,t}$. The group $H_p^{s,t}$, which in our case is also a vector space, consists of classes which exist in $K_s$ and survive until $K_t$. The dimensions of these vector spaces are the \textit{persistent Betti numbers}, denoted $\beta^{s,t}_p$.

An \textit{interval module}, denoted $I=I(b,d)$, is a persistent module of the form
\[ 0 \rightarrow \cdots \rightarrow 0 \rightarrow \Rspace \rightarrow \Rspace \rightarrow 0 \rightarrow \cdots \rightarrow 0.\]
In the above, $\Rspace$ is generated by a homology class and the maps connecting the $\Rspace$s map generator to generator. 
The first $\Rspace$ appears at index $b$ and the last appears at index $d$. 
For any $b \leq r < d$, $I_r = \Rspace$; and for other $r$, $I_r=0$. 
Any persistence module can be decomposed into a collection of interval modules in a unique way \cite{LuoHenselman-Petrusek2023}. 
Consequently, a homology class that lives in time period $[b,d)$ can be written as a linear combination of intervals.
Each interval module is determined by the index of the first $\Rspace$, or the time it is born and the index of the last $\Rspace$ where it dies, which can be $\infty$.
The collection of $[b,d)$ for all interval modules is called the \textit{persistence barcode}. 
When plotted as points in an extended plane, the result is the equivalent \textit{persistence diagram}. 
The persistence barcode therefore contains a summary of the homological changes in the filtration. 

\para{Interleaving and Stability.}
Let $F$ and $G$ be two filtrations over the complexes $K$ and $K'$ respectively, and let the maps connecting the complexes of filtration be $f^{s,t}$ and $g^{s,t}$ respectively, for all $s,t \in \Rspace, s\leq t $. Let $C(F)$ and $C(G)$ be the corresponding filtrations of chain groups, and $H(F)$ and $H(G)$ the corresponding persistence modules. We denote the maps induced on chain groups and homology groups also by $f^{s,t}$ and $g^{s,t}$ respectively, for all $s,t \in \Rspace, s\leq t $.

\begin{definition}
\label{def:chain-interleaving}
Let $F$ and $G$ be two filtrations over the complexes $K$ and $K'$ respectively. 
An \textit{$\eps$-chain-interleaving between $F$ and $G$} (or an $\eps$-interleaving at the chain level) is given by two sets of homomorphisms $\{\phi_\alpha : C(K_\alpha) \xrightarrow{} C(K'_{\alpha+\eps}) \}$ and $\{\psi_\alpha : C(K'_{\alpha}) \xrightarrow{} C(K_{\alpha+\eps}) \}$, such that 
\begin{enumerate}
    \item $\{ \phi_\alpha \}$ and $\{\psi_\alpha \}$ commute with the maps of the filtration, that is, for all $\alpha,t \in \Rspace$, $g^{\alpha+\eps,\alpha+\eps + t} \phi_\alpha = \phi_{\alpha+t} f^{\alpha, \alpha+t}$ and $f^{\alpha+\eps,\alpha+\eps+t} \psi_\alpha = \psi_{\alpha+t} g^{\alpha, \alpha+t}$; 
    \item The following diagrams commute: 
    \begin{equation}
      \begin{tikzcd}
  C(K_\alpha)
    \ar[r,"f^{\alpha, \alpha+\eps}"]
    \ar[dr, "\phi_\alpha", very near start, outer sep = -2pt]
  & C(K_{\alpha+\eps})
    \ar[r, "f^{\alpha+\eps, \alpha+2\eps}"]
    \ar[dr, "\phi_{\alpha+\eps}", very near start, outer sep = -2pt]
  & C(K_{\alpha+2\eps})
  \\
  C(K'_\alpha)
    \ar[r, swap,"g^{\alpha, \alpha+\eps}"]
    \ar[ur, crossing over, "\psi_\alpha"', very near start, outer sep = -2pt]
  & C(K'_{\alpha+\eps})
    \ar[r, swap,"g^{\alpha+\eps, \alpha+2\eps}"]
    \ar[ur, crossing over, "\psi_{\alpha+\eps}"', very near start, outer sep = -2pt]
  & C(K'_{\alpha+2\eps}).
  \end{tikzcd}
    \end{equation}
\end{enumerate}

The \emph{chain interleaving distance} is defined to be 
\begin{equation}
d_{CI}(F, G) := \inf \{\eps\geq 0 \mid \text{there exists an $\eps$-chain interleaving between } F\; \text{and}\; G\}.
\end{equation}
\end{definition}

The standard notion of $\eps$-interleaving~\cite{ChazalCohenSteinerGlisse2009}, denoted $d_I(F,G)$, is defined analogously to our definition above, however, it is defined on the persistence modules $H(F)$ and $H(G)$ on the homology level, rather than the filtration of chain groups.  For our purposes, we require the existence of a chain interleaving. In the application to sublevel set filtrations, which is the main setting in which stability is proved~\cite{cohen2005stability}, the chain interleaving exists, therefore, this strengthening of the interleaving does not hurt the sublevel set stability arguments.

The stability of persistence barcode (or diagram) is a crucial property for applications. It expresses the fact that small changes in data lead to small changes in persistence barcodes. The interleaving distance provides the measure of change in data, and we measure the distance between barcodes using the bottleneck distance. Let $D=Dgm(F)$ and $D'=Dgm(G)$ denote the persistence barcodes (or diagrams) of filtrations $F$ and $G$. 
Recall that the diagram is a multi-set of points and contains all the diagonal points.
The \textit{bottleneck distance} is defined as 
\[
d_B(D, D') = \text{inf}_\gamma \text{sup}_{p \in D} || p - \gamma(p) ||_\infty,
\]
where $\gamma$ ranges over all bijections between $D$ and $D'$ and $||\cdot ||_\infty$ is the largest absolute value of the difference of coordinates, or considered as bars, the largest distortion of an endpoint when matched to the bar of $D'$.   
We refer to~\cite{ChazalCohenSteinerGlisse2009} for the proof of the following \Cref{theorem:persistence-stability}.

\begin{theorem}
\label{theorem:persistence-stability}
    Let $F$ and $G$ be filtrations defined over (finite) complexes $K$ and $K'$, respectively. Then $$ d_B( Dgm(F), Dgm(G)) \leq d_I(F,G).$$
\end{theorem}

Please see~\cite{cohen2005stability, ChazalCohenSteinerGlisse2009} for more on stability. We also mention that in the above theorem we can replace $d_{CI}$ in place of $d_I$, since existence of an $\eps$-chain-interleaving implies existence of an $\eps$-interleaving on the homology level. The resulting theorem would be weaker.

\para{Conventions.}
Since we work with chains and apply boundary and coboundary operators at different times, we write $\delta_t(c)$ and $\partial_t(c)$ to mean the coboundary and boundary of the chain $c$ at time $t$, respectively, where we consider $c$ to be a chain in the final complex $K$ present at time $t$. 
In this paper, we usually omit the subscript of a homology group; we always fix a dimension and do not write it if there is no danger of ambiguity.
Moreover, we use the words persistence barcode and persistence diagram interchangeably. 
A persistence diagram contains all the diagonal points $[0,0)$, and a persistence barcode contains infinite number of intervals of length $0$. 
We use $F$ and $G$ to denote two filtrations over the complexes $K$ and $K'$ respectively, and we denote the maps connecting the complexes of filtration by $f^{s,t}$ and $g^{s,t}$ respectively, for all $s,t \in \Rspace, s\leq t $. We denote the maps induced on chain groups and homology groups also by $f^{s,t}$ and $g^{s,t}$ respectively, for all $s,t \in \Rspace, s\leq t$.


==> sec-homology.tex <==
\section{Homology and Cohomology}
\label{sec:homology}

Let $K$ be a simplicial complex. 
We give the standard orientation to the simplices of $K$. 
That is, we order the vertices of $K$ and assign to any simplex $\sigma \in K$ the ordering of its vertices induced from an ordering of the vertices. 
This is also the ordering used in all our examples. 
From now on, we think of a simplex $\sigma$ to be supplied with the standard orientation. 
We write simplices as an ordered set of vertices, for instance, if $s=v_0v_1\cdots v_{i}$, and $\sigma = \{v_0, v_1, \ldots, v_i \}$ then by convention $s=\sigma$ if the sign of the ordering $v_0v_1\cdots v_{i}$ agrees with the sign of the standard orientation, otherwise $s=-\sigma$.

For any integer $p \geq 0$, the $p$-dimensional \textit{chain group} of $K$ with coefficients in $\Rspace$, denoted $C_p(K)$, is an $\Rspace$-vector space generated by the set of $p$-dimensional (oriented) simplices of $K$. Let $K_p$ denote the set of $p$-simplices of $K$ and $n_p=|K_p|$. By fixing an ordering of the set $K_p$, we can identify any $p$-chain $c\in C_p(K)$ with an ordered $n_p$-tuple with real entries.
For each $p$, we fix an ordering for the $p$-simplices (once and for all), and identify $C_p(K)$ and $\Rspace^{n_p}$. 
The standard basis of $\Rspace^{n_p}$ corresponds (under the identification) to the basis of $C_p(K)$ given by the simplices with standard orientation.

The $p$-dimensional boundary matrix $\partial_p: C_p(K) \rightarrow C_{p-1}(K)$ is defined on a simplex basis element by the formula
\[ \partial (v_0v_1 \cdots v_p)= \sum_{j=0}^{p} {(-1)^q (v_0\cdots v_{q-1}v_{q+1}\cdots v_p) }.\]
In the right hand side above, in the $q$-th term $v_q$ is dropped. The formula guarantees the crucial property of the boundary homomorphism: $\partial_{p} \partial_{p+1} = 0$. This simply means that the boundary of a simplex has no boundary. The sequence $C_p(K)$ together with the maps $\partial_p$ define the \textit{simplicial chain complex} of $K$ with real coefficients, denoted $C_{\bullet}(K)$. The group of $p$-dimensional \textit{cycles}, denoted $Z_p(K)$, is the kernel of $\partial_p$. The group of $p$-dimensional boundaries, denoted $B_p(K)$, is the image of $\partial_{p+1}$. The $p$-dimensional homology group of $K$, denoted $H_p(K)$, is the quotient group $Z_p(K)/B_p(K)$. 
As a set, this quotient is formally defined as $\{z+B_p(K) \mid  z\in Z_p(K)\}$. The operations are inherited from the chain group. In words, the homology group is obtained from $Z_p(K)$ by setting any two cycles which differ by a boundary to be equal. All these groups are $\Rspace$-vector spaces.

Consider the space $\Rspace^{n_p}$. The cycle group $Z_p(K) \subset C_p(K) = \Rspace^{n_p}$ is a subspace, that is, a hyperplane passing through the origin. Similarly, the boundary group $B_p(K)$ is a subspace, and is included in $Z_p(K)$. The homology group is the set of parallels of $B_p(K)$ inside $Z_p(K)$. Each such parallel hyperplane differs from $B_p(K)$ by a translation given by some cycle $z$. These parallel hyperplanes partition $Z_p(K)$. The homology group is then isomorphic to the subspace perpendicular to $B_p(K)$ inside $Z_p(K)$. 
The dimension of the $p$-dimensional homology group is called the $p$-th $\Rspace$-Betti number, denoted $\beta_p(K)$. 

Simplicial \textit{cohomology} with coefficients in $\Rspace$ is usually  defined by the process of dualizing. This means that we replace an $i$-chain by a linear functional $C_p(K) \rightarrow \Rspace$, called a $p$-dimensional \textit{cochain}. 
The set of all such linear functions is a vector space isomorphic to $C_p(K)$, called the cochain group, denoted $C^p(K)$, which is a dual vector space of $C_p(K)$.  
For the purposes of defining harmonic chains, we must fix an isomorphism. 
We take the isomorphism that sends each standard basis element of $\Rspace^{n_p}$, corresponding to $\sigma$, to a functional which assigns 1 to $\sigma$ and 0 to other basis elements, denoted $\hat{\sigma} \in C^p(K)$. Any cochain $\gamma \in C^p(K)$ can be written as a linear combination of the $\hat{\sigma}$. Therefore, it is also a vector in $\Rspace^{n_p}$. The fixed isomorphism allows us to identify $C^p$ with $\Rspace^{n_p}$, and hence to $C_p$. Therefore, any vector in $\Rspace^{n_p}$ is at the same time a chain and a cochain.

The \textit{coboundary matrix} $\delta^p: C^p(K)\rightarrow C^{p+1}(K)$ is the transpose of $\partial_{p+1}$, $\delta^p = \partial_{p+1}^T$. It follows that $\delta_{p+1}\delta_p=0$, and we can form a \textit{cochain complex} $C^{\bullet}(K)$. The group of \textit{$p$-cocycles}, denoted $Z^p$ is the kernel of $\delta^p$. The group of \textit{$p$-coboundary} is the image of $\delta_{p-1}$. The $p$-dimensional \textit{cohomology group}, denoted $H^p(K)$ is defined as $H^p(K) = Z^p(K)/B^p(K)$. All of these groups are again vector subspaces of $C^p(K)$ and thus of $\Rspace^{n_p}$.
It is a standard fact that homology and cohomology groups with real coefficients are isomorphic.

==> sec-stable-barcode-details.tex <==
\section{Proofs Relevant to Canonical Harmonic Chain Barcode}
\label{sec:stable-barcode-details}

We give omitted proofs associated with \cref{sec:stable-barcode}.

\subsection{Proof of \Cref{thm:uniqueness}}
\begin{proof}
We prove a stronger claim below by induction on the dimension of the subspaces of Z(K):
\begin{itemize}[noitemsep,leftmargin=*]
\item 
For each subspace $A \subset Z(K)$, there is a unique set of independent spans of cycles of $A$ realizing a lexicographical maximal (lex.-maximal) sequence of span lengths of cycles of $A$.
\end{itemize}
 
The base case for the induction is to prove the theorem for any subspace $A \subset Z(K)$ of dimension 1. $A$ is generated by any of its non-zero elements $z$. If $\delta(z)\neq 0$, then $\delta(cz)\neq 0$ for all $c\neq 0$. Moreover, if $\partial(d) = z$, $\partial (cd) = cz$. Therefore, all of $A$ either die at the same time or survive until the end. In each case, the spans of all cycles are equal, and there is exactly one span.

Assume the statement is true for all subspaces of dimension at most $m$, and we consider a subspace $A \subset Z(K)$ of dimension $m+1$. For the sake of contradiction, let $I_1, I_2, \ldots$ and $J_1, J_2, \ldots$ be two different sequences of independent spans realizing $\lambda_1, \lambda_2, \ldots$ which is the lex.-maximal sequence of independent span lengths of cycles in $A$. 

Let $k$ be the first index such that $I_k \neq J_k$. Let $\lambda_{l_1}, \ldots, \lambda_{l_s}$ be all the $\lambda_i$ such that $\lambda_{l_j} = \lambda_k$ (for $j=1,\ldots,s$). 
If the two sets of spans $\{I_{l_i}, i =1,\ldots,s \}$ and $\{ J_{l_i}, i=1, \ldots, s \}$ are equal, then, as sets, the two sequences would not differ at spans of length $\lambda_k$. We can therefore assume that these two sets $\{I_{l_i}\}$ and $\{J_{l_i}\}$ are distinct. For each $k$, let $I_k$ be the span of a cycle $x_k$ and $J_k$ be the span of a cycle $y_k$. $\big(x_k\big)$ and $\big(y_k\big)$ are sequences of independent cycles by definition.

We divide the argument into three cases:
\begin{itemize}[noitemsep,leftmargin=*]
\item Case (1) $l_s$ is less than $\dim(A)$. This means that there are independent intervals with length smaller than $\lambda_k$. The subspace $S_x \subset A$ generated by $x_1, \ldots, x_{l_s}$ and $S_y \subset A$ generated $y_1, \ldots, y_{l_s}$ are of dimension at most $m$. Since the sets $\{I_{l_i}, i =1,\ldots,s \}$ and $\{ J_{l_i}, i=1, \ldots, s \}$ are distinct, and these are the only ones of length $\lambda_k$ in the two sequences, the sets $\{ x_{1}, \ldots, x_{l_s} \}$ and $\{y_1, \ldots, y_{l_s}\}$ are distinct. The induction hypothesis implies that $S_x$ and $S_y$ are distinct subspaces of equal dimensions. It follows that at least one of $y_1, y_2, \ldots, y_{l_s}$ is not in $S_x$. Let $y$ be such a cycle. Adding $y$ to sequence $x_1, \ldots, x_{l_s}$ certainly creates a larger lexicographic sequence of lengths of independent cycles. This is a contradiction.   
\item Case (2) $l_s$ equals $\dim(A)$ and $k>1$. In this case, let subspace $S_x \subset A$ be generated by $x_1, \ldots, x_{l_1-1}$ and $S_y \subset A$ be generated $y_1, \ldots, y_{l_1-1}$. If $S_x$ and $S_y$ are distinct subspaces, then at least one of $y_1, \ldots, y_{l_1-1}$, say $y$, would not be in $S_x$. Adding length of span of $y$ to the maximal sequence of independent span lengths will make it larger. It follows that $S_x = S_y$. Therefore, all the spans of length less than $\lambda_k$ in $(I_i)$ and $(J_i)$ are equal as sets. Let $T = \{ span(z) | z \in A ,  z \notin S_x \}$. By our assumption, the sets $\{ I_{l_1}, \ldots, I_{l_s} \}$ and $\{ J_{l_1}, \ldots, J_{l_s} \}$ are two distinct subsets of $T$. If they generate the same subspace, the subspace would be of dimension at most $m$, and they have to be equal, by the induction hypothesis, since they realize the same maximal span-length sequence, namely $l_s$ copies of $\lambda_k$. Hence, they generate distinct subspaces which again leads to a contradiction similar to Case (1).
\item Case (3) $l_s$ equals $\dim(A)$ and $k=1$. The spans of length $\lambda_k$ create all of $A$ and all the $\lambda_i$'s are equal. The two sequences $\big(x_k\big)$ and $\big(y_k\big)$ give two sets of basis elements for $A$, all having equal span-lengths. Let $x$ be a cycle with smallest birth time whose interval is not among $\big(J_i\big)$. Let $t$ be the time $x$ is generated. If no $y_k$ is generated at $t$, then $x$ is independent of all $y_k$ which is a contradiction. Therefore some $y_k$, say $y$, is generated at time $t$. Since $span(x)$ has the same length as $span(y)$, it follows that $span(x) = span(y)$, and we reach a contradiction with the choice of $x$. 
\end{itemize}
\end{proof}

\subsection{Proof of \Cref{{lemma:box-lemma}}}

\begin{proof}
In the following argument by a chain $c_t$ we mean the chain $c$ of $K$ considered as a chain of $K_t$. \cref{fig:boxlemma} helps the argument.
Consider the chain $z'=\phi_\alpha(z)$. $z'$ is clearly a cycle and since the maps are harmonic preserving, and $f^{\alpha,\alpha+2\eps}(z) \in Z_{\alpha+2\eps}(K)$ is still a cocycle, by the harmonic preserving property $z'$ is a cocycle and hence harmonic. We now consider the span of $z'$ in $G$, let it be denoted by $[\alpha', \beta')$. 

We have seen already that $\alpha'-\alpha \leq \eps$. Assume, for the sake of contradiction, that $\alpha - \alpha '>\eps$. Then $z'$ exists at time $\alpha-\eps-\eta$ for small $\eta$. We consider $y = \psi_{\alpha-\eps-\eta} (z'_{\alpha-\eps-\eta}) \in F_{\alpha-\eta}$. We suppress the $x$ in $f^{x,y}$ in the coming calculations, it can be deduced from the argument. We also suppress the subscripts of $\phi_t, \psi_t$. 

We have 
\[  f^{2\eps+\eta} (y) = f^\eta \psi \phi (y) = \psi g^\eta \phi(y) = \psi g^\eta \phi \psi (z'_{\alpha-\eps-\eta}) = \psi g^{2\eps+\eta} (z'_{\alpha-\eps-\eta}) = \psi(z'_{\alpha+\eps}) = z_{\alpha+2\eps}. \] 
Since $f$ is the inclusion, it follows that $y = z_{\alpha-\eta}$ which is a contradiction since $z$ does not exist at $\alpha-\eta$. It follows that $ \alpha-\alpha' \leq \eps$.

If $\beta'-\beta>\eps$, then $|span(z')|>\eps$ by the argument on starting points of $span(z')$ above. We can deduce that $\psi(z'_{\beta'-\eps}) = z_{\beta'}$ is harmonic by the harmonic preserving property of $\psi$. This is a contradiction since the interval of $z = \psi(z') = \psi\phi(z)$ ends at $\beta < \beta'-\eps$. Therefore, $\beta'-\beta \leq \eps$.

Assume $\beta-\beta'>\eps$. Then for small $\eta>0$, $\beta-\eps-\eta > \beta'$. It follows that $\phi(z_{\beta-\eps-\eta}) = z'_{\beta-\eta}$ is harmonic which is a contradiction, since $z'_{\beta'}$ is not harmonic and the maps are inclusions.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{boxlemma.pdf}
    \caption{A schematic for the proof of~\Cref{lemma:box-lemma}.}
    \label{fig:boxlemma}
\end{figure}

\subsection{Proof of \Cref{lemma:simple-stability}}


\begin{proof}
Let $I_1, I_2, \ldots, I_{p_F}$ be the sequence of the intervals of $F$ in the canonical {\hcb}, and $J_1, J_2, \ldots, J_{p_G}$ be those of $G$. Moreover, let $d_1, d_2, \ldots, d_{q_F}$ be distinct lengths of the intervals $I_i$, and $l_1,l_2, \ldots, l_{q_F}$ be the lengths for $G$, in order. Let $\{ \phi_t \}$, $\{ \psi_t \}$ define a harmonic-preserving $\eps$-interleaving between $F$ and $G$, where $\eps$ is arbitrarily close to $d_{HI}(F,G)$. 


Let the subspace $\Lambda_j \subset Z(K)$ be generated by cycles $z_i$ associated to $I_i$ with $|I_i| \leq  d_j$. Similarly, let $\Lambda'_j \subset Z(K')$ be the subspace generated by cycles $y_i$ associated to $J_i$ with $|J_i| \leq l_j$. We claim that for all $j$, if $d_j > 2\eps$ or $l_j > 2\eps$ then $\phi(\Lambda_j) = \Lambda'_j$  and we can match intervals of length at least $d_j$ to those of at least $l_j$.  

In the following for any cycle $z \in Z(K)$, by $\phi(z)$ we mean $\phi_\alpha(z)$ where $\alpha$ is the time that $z$ is born. We extend this convention to subspaces of cycles in the natural way. 
We first prove the claim for $j=1$. Without loss of generality, assume $ d_1 \geq l_1 $. Consider a generator $z$ of $\Lambda_1$ associated to an interval with length $d_1$. If $\phi(z) \notin \Lambda'_1$, then, \Cref{lemma:box-lemma} implies that we can add one more independent span length of length at least $ d_1 - 2\eps  \geq l_1- 2\eps \geq l_1 -\delta(G)/2 > l_2$ to the lex-maximal independent span length sequence of $G$. This is a contradiction. It follows that $\phi(\Lambda_1) \subset \Lambda'_1$. To show that $\Lambda'_1 \subset \phi (\Lambda_1)$, it is enough to argue that the generators of $\Lambda'_1$ are in the image. Since $\phi(\Lambda_1) \subset \Lambda'_1$ we have $d_1 \geq l_1 - 2\eps$. If one such generator $y$ is not in the image $\phi(\Lambda_1)$, then $|span(\psi(y))| \geq l_1 - 4\eps > d_2$, hence $\psi(y) \in \Lambda_1$. Thus $y = \phi \psi (y) \in \Lambda'_1$. This contradicts our assumption on $y$. It follows that $\lambda'_1 \subset \phi(\Lambda_1)$ and thus $\Lambda'_1 = \phi(\Lambda_1)$. 

We now show that each interval $I_i$ in the barcode of $F$ with $|I_i| = d_1$, has to be mapped by $\phi$ to an interval with length $l_1$ in the barcode of $G$. Let an interval $I$ be generated by $z$. Since $\phi(z) \in \Lambda'_1$, $\phi(z)$ can be written as a combination of generators $y_1, \ldots, y_{n_1}$ of intervals of the barcode of $G$. $\phi(z)$ has to be born at the time when one of the $y_i$ is born. It follows that $span(\phi(z))$ agrees with interval of $y_i$, since the start and end of the next nearest interval differs by at least $\delta(G)> \eps$ from start and end of interval of $\phi(z)$.

Assume we have matched the intervals of length less than $d_k$ to those of length less than $l_k$ and such that the endpoints of matched intervals are within $\eps$. We consider the intervals of length $d_k$ and $l_k$. Without loss of generality assume $d_k > l_k$. Let $z$ be a generator of length $d_k$. Since $\phi$ is injective $\phi(z)$ is independent of $\Lambda'_{k-1}$. If $d_k > l_k + 2\eps$ then the lex-maximal sequence of span lengths of $G$ can be improved by adding $\phi(z)$. Therefore, $\phi(\Lambda_k) \subset \Lambda'_k$ and $d_k \leq l_k+2\eps$ and $l_k \geq d_k -2\eps$. 
If there is a $y \notin \phi(\Lambda'_k)$ which is a generator of an interval $J_i$ of length $l_k$, then $span(\psi(y))$ is of length at least $l_k -2\eps \geq d_k-4\eps = d_k -\delta(F)$. The next span length is at most $d_k-\delta$. Therefore, $|span(\psi(z))|=d_k$ and $\psi(y)$ needs to be in $\Lambda_k$, and we reach a contradiction as before.  It follows that $\phi(\Lambda_k) = \Lambda'_k$.   

We now show that each interval $I_i$ in the barcode of $F$ with $|I_i| = d_k$, has to be mapped by $\phi$ to an interval with length $l_k$ in the barcode of $G$. Let intervals $I_1, \ldots, I_m$ of length $d_k$ be generated by $z_1, \ldots, z_m$. For each $i$, since $\phi(z_i) \in \Lambda'_k$, $\phi(z_i)$ can be written as a combination of generators $y_1, \ldots, y_{n_k}$ of intervals of the barcode of $G$ of length up to $d_k$. $\phi(z_i)$ has to be born at the starting point of some $y_{j_i}$ in the combination, say at time $t_i$. By induction hypothesis, all intervals of length longer than $l_k$ born at $t_i$ are already matched, so at time $t$ an interval of length at most $l_k$ is generated for each $i=1,\ldots,m$, otherwise, some of $\phi(z_i)$ would be in $\Lambda'_{k-1}$. Since $l_{k+1}-l_k> \delta$, it follows that an interval of length $l_k$ is generated at time $t_i$, and we can match $span(z_i)$ with some interval of length $l_k$ in the barcode of $G$ with a cost of $\eps$.

The above argument can be repeated as long as both $d_k$ and $l_k$ are present, and $\min{d_k,l_k} > \eps$ so that we can use the harmonic-preserving property of the interleaving maps. By~\Cref{lemma:box-lemma}, if $\max\{d_k, l_k\}> 2\eps$, then $\min\{l_k,d_k\}>\eps$. So the argument can be repeated as long as $\max\{d_k, l_k\} > 2\eps$. If $\max\{d_k, l_k\} \leq 2\eps$ we match the interval to the nearest point of the diagonal. This is possible again with a cost of $\eps$.
\end{proof}

\subsection{Proof of \Cref{theorem:interpolation}}

\begin{proof}
The proof is based on the argument of~\cite{cohen2005stability} with some modifications. Let $c = ||\hat{f} -\hat{g}||_\infty$. We define a 1-parameter family of convex combinations $h_\lambda = (1-\lambda)\hat{f} + \lambda\hat{g}$, $\lambda \in [0,1]$. These functions interpolate $\hat{f}$ and $\hat{g}$. Since $K$ is finite, the images $\hat{f}(K)$ and $\hat{g}(K)$ are bounded. Without loss of generality, we assume that values are at least 1 and 
$\hat{f}(x), \hat{g}(x) < M$ for all $x$. 

Given a convex combination of the form $h_\lambda = (1-\lambda)\hat{f} + \lambda\hat{g}$, $\delta(\lambda):=\delta(h_\lambda)$ is positive, and we have $h_\lambda < M$. The set $C$ of open intervals $J_\lambda = \left(\frac{\lambda - \delta(\lambda)}{(1+M)4c}, \lambda + \frac{\delta(\lambda)}{(1+M)4c}\right)$ forms an open cover of $[0,1]$. Since $[0,1]$ is compact, $C$ has a finite sub-cover defined using $\lambda_1 < \lambda_2 < \ldots < \lambda_n$ such that each two consecutive intervals $J_{\lambda_i}$ and $J_{\lambda_{i+1}}$ intersect. Then,
\begin{center}
\begin{align}
\begin{split}
     \lambda_{i+1} - \lambda_i & \leq \frac{(\delta(\lambda_i)+\delta(\lambda_{i+1}))}{(1+M)4c}  \\
     & \leq \frac{\min\{\delta(\lambda_i), \delta(\lambda_{i+1})\}(1+M)}{(1+M)4c} \\
     & \leq \frac{\min\{\delta(\lambda_i),\delta( \lambda_{i+1})\}}{4c}.
\end{split}     
\end{align}
\end{center}

Since $c = ||\hat{f} -\hat{g}||_\infty$, $||h_{\lambda_i} - h_{\lambda_{i+1}} ||_\infty = c(\lambda_{i+1}-\lambda_i)=: c_\lambda.$ It follows that $||h_{\lambda_i} - h_{\lambda_{i+1}} ||_\infty \leq \min\{\delta(\lambda_i),\delta(\lambda_{i+1})\}/4.$

Let $F(\lambda_i)$ denote the sublevel set filtration of $h_{\lambda_i}.$
Since the filtrations are sublevel set filtrations of the same complex, we have that $F(\lambda_i)_{\alpha} \subset F(\lambda_{i+1})_{\alpha+c_\lambda}$, and $F(\lambda_{i+1})_\alpha \subset F(\lambda_i)_{\alpha+c_\lambda}$. Since the inclusion is harmonic-preserving, we deduce 
\[d_{HI}(F(\lambda_{i+1}),F(\lambda_{i})) \leq ||h_{\lambda_i} - h_{\lambda_{i+1}} ||_\infty = c(\lambda_{i+1}-\lambda_i) \leq \frac{\min\{\delta(\lambda_i),\delta(\lambda_{i+1})\}}{4c}.\]
It follows from~\Cref{lemma:simple-stability} that $$d_B(\chd(F_{\lambda_i}), \chd (F_{\lambda_{i+1}})) \leq d_{HI}(F(\lambda_i),F(\lambda_{i+1})) \leq ||h_{\lambda_i} - h_{\lambda_{i+1}}||_\infty.$$

The concatenation of these inequalities follows the proof of Interpolation Lemma in~\cite{cohen2005stability} verbatim leading to the statement of the theorem.
\end{proof}



==> sec-stable-barcode.tex <==
\section{Canonical Harmonic Chain Barcode and Stability}
\label{sec:stable-barcode}

Fix a homological dimension $p$ and consider a filtration $F$ and a homology class $h \in H_p(K_b)$ born at time $b$ which dies at time $d$ when entering $K_d$. 
The rank (dimension) of $p$-th homology group increases at time $b$. The class $h$ contains a unique harmonic cycle $z$. We say that the harmonic cycle $z$ is \emph{born} at time $b$. When a persistent homology class dies (i.e., becomes a boundary), then clearly the corresponding harmonic cycle also \emph{dies}. Contrary to the ordinary persistent homology, this is not the only situation where a harmonic cycle dies. 
In brief, a harmonic cycle dies whenever it bounds a chain or gets a non-zero coboundary. 
A crucial property, which is not hard to verify, is that when a cycle is no longer a cocycle, it could never become a cocycle in the future. Moreover, when a harmonic cycle dies, it is because a relation is introduced in homology (i.e. a homology class dies); the classes then change their harmonic representatives.  

Recall that the space of harmonic $p$-cycles at time $t$, which we denote $\har_p(K_t)$, is isomorphic with the $p$-th homology $H_p(K_t)$. A cycle might be a harmonic cycle when it is first created, and then it might fail to be harmonic at a later time: for example, it might get a non-zero coboundary,  or become a boundary. Alternatively, it may remain harmonic up to infinity. 
When working with cycles, we usually fix a dimension $p$ and  suppress the dimension in the notation $H:=H_p, Z:=Z_p$, etc. 
Moreover, for simplicity of exposition, we treat $\infty$ as a fixed large number, so that all our interval lengths can be compared to each other. See \cref{sec:stable-barcode-details} for omitted proofs. 

\begin{definition}
\label{def:span}
For a cycle $z \in Z(K)$, its \emph{harmonic span}, denoted $span(z)$, is an interval of the form $[s,t)$ in the filtration during which $z$ is a (non-trivial) harmonic cycle. 
If a cycle is non-harmonic at birth, its span is empty and has length $0$. If a cycle is harmonic in $K$, its span has length $\infty$. The length of a span is denoted by $|span(z)|$.   
\end{definition}

\Cref{def:span} assigns an interval to each cycle of the final complex $K$. This would be an assignment of an interval to each vector in a $\Rspace$-valued vector space. When talking about independence of cycles, we always consider them as vectors in the cycle space $Z(K)$. 

\begin{definition}
\label{def:independent-cycles}
Let $\big(z_i\big):=z_1,z_2,\ldots \in Z(K)$ be a (finite) sequence of cycles. 
We say $\big(z_i\big)$ is a \emph{sequence of independent cycles} if, for each $i>1$, $z_i$ does not belong to the subspace generated by $z_1, \ldots, z_{i-1}$ in $Z(K)$. 
If $\big(z_i\big)$ is a sequence of independent cycles, the sequence 
$\big(span(z_i)\big): =span(z_1), span(z_2), \ldots$ is called a sequence of \emph{independent spans}, and the sequence 
$\big(|span(z_i)|\big):= |span(z_1)|, |span(z_2)|, \ldots$ is called a sequence of \emph{independent span-lengths}.  
The set of spans forming a sequence of independent spans is called a \emph{set of independent spans}.
\end{definition}

The number of cycles in a sequence of independent cycles equals the dimension of $Z(K).$
A sequence of independent span-lengths is a sequence of real numbers. We can compare any two sequences using the lexicographic ordering, starting from the first number in the sequence. 
That is, if $S_1 = \big(|span(z_i)|\big)$ and $S_2 =  \big(|span(y_i)|\big)$ are two sequences of independent span-lengths, we say $S_1 > S_2$ if and only if there is an index $k$ such that for all $j<k$, $|span(z_i)|=|span(y_i)|$, and $|span(z_k)| > |span(y_k)|$.  

\begin{theorem}
\label{thm:uniqueness}
    Let $\big(\lambda_i\big) = \lambda_1, \lambda_2, \ldots $ be the sequence of independent span lengths which is lexicographical maximal. Then there is a unique set of independent spans $\{J_1, J_2, \ldots\}$ whose sequence of lengths equals $\big(\lambda_i\big)$.  
\end{theorem}
\noindent \Cref{thm:uniqueness} allows us to define the \emph{canonical barcode of harmonic chains}  unambiguously as follows.

\begin{definition}
\label{def:chcb}
Given a filtration $F$, the set of spans realizing the lexicographical maximal sequence of independent span lengths is called the \emph{canonical barcode of harmonic chains} (equivalently, the \emph{canonical diagram of harmonic chains}), denoted as $\chd(F)$. 
\end{definition} 
Given any filtration $F$, \Cref{def:chcb} associates a unique barcode to $F$. And this barcode is, in general, distinct from a persistence barcode.
For now on, canonical harmonic chain barcode (or simply,  {\hcb}) means canonical barcode of harmonic chains. 

\subsection{Example 1}
\cref{fig:c-harmonic-example} depicts a $1$-dimensional canonical barcode of harmonic chains, from the example in~\cref{fig:first-attempt-example}. 
At time $9$, the first cycle $r_1 = 7+8-9$ is created. 
This event creates a harmonic bar that ends at $t_1$ when $r_1$ gets a coboundary. 
At time $11$, a second cycle $r_2$ is created, leading to an increase in the dimension of $Z(K_{11})$. 
To compute a cycle that survives the longest, we start from $t=+\infty$ and compute the largest $t$ such that $Z(K_{11}) \cap \har(K_t) = Z(K_{11}) \cap \ker (\delta_t) \neq \{ 0 \}$. Take the cycle $r_2 = 7+8+10-11$. $r_2$ is harmonic, and it survives up until $t_3$. 
One can check that if a cycle has non-zero coefficient for $9$, it has to die earlier; therefore, $r_2$ represents the longest bar generated at $11$, namely, $[11,t_3)$. 
At time $13$, similar to time $11$, we obtain a cycle $r_3$ which represents a bar $[13,t_2)$. 
Now, at time $15$, we have all possible edges so there has to be a harmonic chain that survives up to $t_4$. We take $r_4 = 3r_1 - \partial( t_1+t_2+t_3)$. One checks easily that $\delta_t \partial (r_j) = \delta_t(9)$, for $j=2,3,4$. Therefore, $\delta_t(r_4) = 3\delta_t(9)-3\delta_t(9)=0$ for $ 15 \leq t < t_4$. 

\begin{figure}
    \centering
    \includegraphics[scale=.85]{c-harmonic-example.pdf}
    \caption{The canonical {\hcb} (in blue) for the filtration  in~\cref{fig:first-attempt-example}.}
    \label{fig:c-harmonic-example}
\end{figure}

\subsection{Example 2}
We provide a second example which sheds more light on the nature of the canonical {\hcb}. In this example, we have two filtrations $F_1$ and $F_2$ of the same underlying complex $K$. We are only interested in the 1-dimensional homology. In $F_1$, two independent 1-dimensional  homology classes are born early in the filtration, then cycles of low persistence are created and immediately killed. At the end, the two independent cycles created at the start are also killed. 

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.8]{example-2a.pdf}
    \caption{The ordinary persistence barcode and the canonical barcode of harmonic chains for the filtration $F_1$. (a) The insertion times of of edges and triangles.  (b) The 2-dimensional boundary matrix, the matrices of different times steps are marked. (c) The ordinary persistence barcode (in black). (d) The canonical barcode of harmonic chains (in blue).}
    \label{fig:example-2a}
\end{figure}

The first filtration $F_1$ is shown in~\cref{fig:example-2a}. 
Its ordinary persistence barcode is shown in (c), and its canonical {\hcb} is shown in (d). 
We see that, in the ordinary persistence barcode in (c), the two 1-dimensional homology classes that are created at the beginning give rise to two long bars, whereas other cycles create short bars. 
Contrary to the ordinary persistence barcode, we see that all the harmonic bars in the canonical {\hcb} (d) are rather short.

In~\cref{fig:example-2b}, we consider a second filtration $F_2$. 
In this filtration, first all the edges are inserted and then all the triangles. 
The canonical {\hcb} is justified since at the time when the last edge is inserted, already all the harmonic chains are present, and at the insertion of a triangle, the dimension of harmonic chains decreases by 1. 
Therefore, one can find harmonic chains that survive the insertion of triangles.

\subsection{Comparison: Persistence Barcode vs. Canonical Harmonic Chain Barcode}  
In the filtration $F_1$, we see that the canonical barcode of harmonic chains contains short bars whereas the ordinary persistence barcode has long bars. 
Our suggestion of taking canonical {\hcb} does not lead to salient cycle features for this example. 
This reflects the fact that the status of cycles, as being harmonic or not, in the first filtration $F_1$ does not provide us with a feature that spans a long time interval. 


%\Bei{Meaning? This does not rule out, of course, the existence of other types of a stable cycle barcode that in $F_1$ also provides us with a stable barcode with long bars.} 

We observe that the canonical {\hcb} for $F_2$ reflects the existence of geometric features that survive the insertion of many triangles, whereas, the ordinary persistence barcode captures only two long features, if the shorter bars in the persistence barcode of~\cref{fig:example-2b} are considered as noise. 
Therefore, we see that the canonical {\hcb} can differentiate these two situations, whereas the ordinary persistence  barcode cannot (again, if we consider the shorter bars in the ordinary persistence barcode as noise).   

\subsection{Computing Canonical Barcode of Harmonic Chains}
\label{ssec:computation}

To compute the canonical barcode of harmonic chains, we make use of the following algorithm.
Let $F$ be a filtration and $\har(K_i)$ be the harmonic chain group of the complex $K_{t_i}$.

For $i = 0, 1,2, \ldots,m$, let $\chd_{i-1}$ be the part of the barcode computed up to time step $i$, with $\chd(-1) = \emptyset$. For each $j = i+1, i+2, \ldots$ compute $r_{ij} := dim (f^{i,j}(\har(K_{t_i})) \cap \har(K_{t_j}))$, where here we write again $f$ for the induced map on cycles. If there are already $m_i$ bars of $\chd_{i-1}$ alive at time $i$, and $h_i = dim(\har(K_{t_i})$, we add $\max\{h_i - m_i,0\}$ new bars to $\chd_{i-1}$ starting at $i$. These bars will die when $r_{ij}$ decreases as $j$ increases. If at an index $j$, $r_{ij} - r_{ij-1} >0$, we kill $r_{ij} - r_{ij-1}$ many harmonic bars which started at $i$. The bars we do not kill survive to $+\infty$. 
This concludes the description of the algorithm.

This computation can be done easily by first computing for each $i$, the Laplacian and a basis for the nullity of the Laplacian.  
Then for each $j>i$, we compute the matrix of images $\har^{i,j} := f^{i,j}(\har(K_{t_i}))$ simply by appending 0's to the end of a matrix of basis of $\har(K_{t_i})$ to make the number of rows equal to that of the matrix at time $j$. 
We then compute $r_{ij} = dim (f^{i,j}(\har(K_i)) \cap \har(K_j))$ by computing the rank of $ [ \har_j , \har^{i,j}]$ (i.e., the concatenation of two matrices) as an intermediate step. 

If $n$ is the number of simplices in the complex, and $m$ is the number of time steps, then all of these matrix operations can be done in time $O(m^2n^\omega + mn^3)$, where $n^\omega$ is the matrix multiplication time. In the algorithm, we compute the Laplacian and a basis for its kernel in with $n^3$ time in each time step, which is $O(mn^3)$ for all time steps. Then we need for each pair $i<j$, to compute the rank of $ [ \har_j , \har^{i,j}]$, which is possible in $m^2 n^\omega$ time. In total, we have $O(m^2n^\omega + mn^3)$. It is plausible that the runtime can be further improved. Providing the most efficient algorithm to compute the canonical {\hcb} is left for future work. We also prove that this algorithm is correct, see~\cref{sec:correctness} for details. 

\begin{theorem}
    Given a filtration of a complex of size $n$, with $m$ time-steps, we can compute the canonical barcode of harmonic chains in $O(m^2n^\omega + mn^3)$ time.
\end{theorem}


\begin{figure*}[!ht]
    \centering
    \includegraphics[scale=0.8]{example-2b.pdf}
    \caption{The ordinary persistence barcode and the canonical barcode of harmonic chains. (a) The insertion times of edges and triangles for the filtration $F_2$. (b) The 2-dimensional boundary matrix, the matrices of different times steps are marked. (c) The ordinary persistence barcode (in black). (d) The canonical barcode of harmonic chains (in blue). The persistence reduction of the boundary matrix remains the same since the matrix is unchanged. The basis for ordinary persistence barcode therefore remains the same chains as our first ordering, however, the insertion times of simplices are changed, resulting in different bars.}
    \label{fig:example-2b}
\end{figure*}



\subsection{Stability}
We express the stability of the canonical barcode by considering the typical setting in which the two filtrations $F$ and $G$ are sub-level set filtrations for two simplex-wise linear functions $\hat{f}$ and $\hat{g}$, respectively, defined on the same complex $K$. This is the same setting as the seminal stability result of~\cite{cohen2005stability}. However, we prove, as an intermediate step, a more general result. The proofs are inspired by the overall approach of \cite{cohen2005stability}. Similar to~\cite{cohen2005stability}, our stability result can be extended to functions on topological spaces, however, we limit our scope of discussion to simplicial complexes.

We start by defining the notion of harmonic interleaving distance. Then we show that the bottleneck distance between canonical {\hcbs} is upper bounded by the harmonic interleaving distance between the two filtrations; see~\cref{fig:h-interleaving}. Eventually we show that bottleneck distance is upper bounded by $||\hat{f} - \hat{g} ||_\infty$.


\begin{definition}
    Let $\{\phi_\alpha\}$,$\{ \psi_\alpha\}$, $\phi_\alpha: F_\alpha \xrightarrow{} G_{\alpha + \eps}$, $\psi_\alpha: G_\alpha \xrightarrow{} F_{\alpha + \eps}$ be a family of chain maps defining an $\eps$-chain interleaving between $F$ and $G$. We say that the pair of families $\{\phi_\alpha\}$, $\{\psi_\alpha\}$ are \textit{harmonic-preserving} if
    \begin{itemize}[noitemsep,leftmargin=*]
        \item For any harmonic chain $c\in F$, for all $\alpha$ and $\rho \geq \eps$, if $\delta(f^{\alpha, \alpha+ \rho}(c))=0$ then $\delta \phi_\alpha (c)=0$.
        \item For any harmonic chain $c'\in G$, for all $\alpha$ and $\rho \geq \eps$, if $\delta(g^{\alpha,\alpha+\rho}(c'))=0$ then $\delta \psi_\alpha (c')=0$.
    \end{itemize} 

    The harmonic interleaving distance $d_{HI}$ is defined analogously to the chain interleaving distance, however, we allow only harmonic-preserving maps.
\end{definition}


\begin{figure}[!ht]
    \centering
    \includegraphics{hinterleaving.pdf}
    \caption{Harmonic interleaving at the chain level. If $z_\alpha$ is still harmonic at time $\alpha+\rho$, then $\phi(z)$ is harmonic.}
    \label{fig:h-interleaving}
\end{figure}

The following lemma is analogous to the Box Lemma in~\cite{cohen2005stability}; see~\cref{sec:stable-barcode-details} for its proof. 

\begin{lemma}
\label{lemma:box-lemma}
Let $F$ and $G$ be filtrations of complexes $K$ and $K'$, respectively, defined using inclusion maps, and let $\eps > 0$ be such that there are $\{ \phi_t \}$ and $\{ \psi_t \}$ realizing a harmonic-preserving $\eps$-interleaving (at the chain level). Let $z \in Z(K)$ be a cycle with $span(z) = [\alpha, \beta)$ such that $\alpha - \beta > \eps$. Then, writing $[\alpha', \beta')$ for $span((\phi(z)))$ we have $\alpha-\eps \leq \alpha' \leq \alpha+\eps$, and $ \beta -\eps \leq \beta' \leq \beta+\eps.$ 
\end{lemma}



For a filtration $F$, let $\delta(F) = min\{ t_{i+1} - t_{i}, i = 1, \ldots, m-1 \}$. We say that $F$ is \textit{very close} to $G$ if $d_{HI}(F,G) < \min \{ \delta(F)/4, \delta(G)/4 \} $.
Observe that $\delta(F)$ is the minimum possible distance between any two endpoints of intervals or interval lengths.

\begin{lemma}
\label{lemma:simple-stability}
If $F$ is very close to $G$ then
$$ d_B(\chd (F), \chd (G)) \leq d_{HI}(F,G).$$
\end{lemma}

The following is analogous to the Interpolation Lemma from~\cite{cohen2005stability}.

\begin{theorem}
\label{theorem:interpolation}
Let $\hat{f}$ and $\hat{g}$ be two real-valued simplex-wise linear functions defined on a simplicial complex $K$. Let $F$ and $G$ be the sublevel-set filtrations of $\hat{f}$ and $\hat{g}$. Then $$ d_B (\chd(F),\chd(G)) \leq || \hat{f} -\hat{g}||_\infty.$$
\end{theorem}

\subsection{Stability Example}

We consider the same example we presented for instability, see~\cref{fig:stableexample}. 
For the left filtration, at time $t_4$, the cycle $z_1 = t_4+t_2-t_1$ is created and represents the top bar. 
At time $t_5$ the dimension of the harmonic chains increases, and one can see that the cycle $z_2 = t_2-t_1+t_3-t_5$ is harmonic at $t_5$ and survives up to $t_9$.
Among the cycles that exist at $t_5$, a 1-dimensional subspace survives $t_8$, this space is generated by $z_2$.
At $t_7$, all edges are present, therefore there has to be a cycle that survives until $t_{10}$. 
We see that $z_3 = \partial(t_{10}) - 1/2 \partial (t_8 - t_9 )$ has this property and serves as the harmonic representative.

For the right filtration, at time $t_4$, the cycle $\bar{z}_1 = -t_1+t_2+t_4-t_3$ is created and survives up to $t_9$. 
At time $t_5$, $\bar{z}_2 = t_5+t_4-t_3$ is created and  survives up to $t_8$. 
Finally, at time $t_7$, $\bar{z}_3=z_3$ is created and survives up to $t_{10}$.

We observe that the first bar on top on the left can be matched to the second bar on the right, and the second bar in the left can be 
matched to the first bar on the right. The bottom bar is unchanged in both barcodes.

\begin{figure}
    \centering
    \includegraphics{stable-example.pdf}
    \caption{The canonical barcodes of harmonic chains (in blue) are stable.}
    \label{fig:stableexample}
\end{figure}

==> sec-unstable-barcode-details.tex <==
\section{Technical Details on Our First Attempt}
\label{sec:unstable-barcode-details}

We describe technical details in our first attempt in constructing a harmonic chain barcode following \cref{sec:unstable-barcode}.

\subsection{Details on Example in \cref{fig:first-attempt-example}}
Following the filtration given in~\cref{fig:first-attempt-example}(a), the 1-dimensional persistence barcode tracks the births and deaths of 1-cycles. After all vertices and edges have been inserted at time $15$, the triangles $t_1$, $t_2$, $t_3$, and $t_4$ destroy the 1-cycles created at time $15$, $13$, $11$, and $9$, respectively. This gives rise to a persistence barcode (in black) that consists of intervals \update{$B_1=[15,t_1),B_2=[13,t_2),B_3=[11,t_3),B_4=[9,t_4)$}, respectively, shown in~\cref{fig:first-attempt-example}(c).  
\update{After matrix reduction in~\cref{fig:first-attempt-example}(b), 
$B_1$ is represented by the 1-cycle $z_1=9+14-15$, 
$B_2$ is represented by $z_2=13-12+9$,
$B_3$ is represented by $z_3 = 9+10-11$, 
and $B_4$ is represented $z_4 = 7+8-9$.}

To obtain harmonic bars (in purple) we sweep from left to write. 
Right before time $t_1$, $z_i$ also serve as the harmonic representatives.  
At time $t_1$, all of the basis cycles $z_i$ get a coboundary from the triangle $t_1$. 
The homology class of \update{$z_1$} becomes trivial as it is destroyed by the triangle $t_1$, whereas other three homology classes remain non-trivial. 
As the first harmonic bar we observe, $B_1^1 = [15, t_1)$ is identical to the persistence bar $B_1$ and it is represented by a harmonic 1-cycle \update{$z_1^1=z_1$}. 
Now, if we take the cycle representative \update{$z_4$}, the homology class it represents remains non-trivial at time $t_1$, whereas the harmonic 1-cycle $z_4^1=z_4$ has been destroyed creating a harmonic bar $B_4^1=[9,t_1)$.   
We then need to find a new harmonic cycle in its homology class, by finding $x$ such that \update{$\delta(z_4 + \partial x) =0$} at time $t_1$. 
This implies $\delta(z_4) = - \delta \partial x$. 
Since only triangle $t_1$ exists at this time, $\delta(z_4) = \delta(7+8-9) = \delta(7)+\delta(8)- \delta(9) = 0+0-t_1=-t_1.$ 
We also have $\delta \partial t_1 = \delta(15-14+9) = \delta(15)-\delta(14)+\delta(9) = t_1 + t_1 + t_1 = 3t_1$. 
Therefore we can set $x = \frac{1}{3} (t_1)$. 
Then the new harmonic chain is $z^2_4 = z_4 + \frac{1}{3} \partial (t_1)$. 
Similarly, persistence bars $B_2$ and $B_3$ are split at time $t_1$, giving rise to harmonic bars with representatives $z^2_2 = z_2 - \frac{1}{3} \partial (t_1)$ and $z^2_3 = z_3 - \frac{1}{3} \partial (t_1)$. 

At time $t_2$, \update{$z_2^2$} dies as it is destroyed by the triangle $t_2$. 
\update{$z_4^2$} gets a coboundary $-t_2$ and $\delta t_1$ gets a coboundary $t_2$, hence $\delta (z_4^2) = -\frac{2}{3} t_2$. 
A new harmonic cycle is $z_4^3 = z_4 + \frac{1}{4}(\partial t_1 + \partial t_2)$. %\Bei{why?} 
Similarly, $z_3^2 = z_2 - \frac{1}{4}(\partial t_1 + \partial t_2)$. 
At time $t_3$, the cycle $z_3^3$ and its harmonic homologous cycles die. $z_4^3$ also becomes non-harmonic and will be replaced by another harmonic cycle that will die at $t_4$.

\subsection{Details on Example in \cref{fig:instability}}

\cref{fig:instability} shows two filtrations whose only difference is the exchange of times when edges $12$ and $23$ are inserted. 
In this example, vertices are labeled 1 to 5, and higher-dimensional simplices (edges and triangles) are labeled by $t_i$ (for some $i$). 
That is, edges appear at times $t_1$ to $t_7$, and triangles appear at times $t_8,t_9$ and $t_{10}$, respectively. 
The persistence barcodes are shown in black. 
The unstable {\hcbs} constructed from our first attempt using the basis given by the standard matrix reduction algorithm are shown in purple. 

In the left filtration, the matrix reduction algorithm for persistence homology gives the following cycle representatives,   
$z_1 = -t_1+t_2+t_4$, 
$z_2 = -t_3+t_4+t_5$,
and $z_3=t_4-t_6+t_7$, 
for persistence bars $B_1$, $B_2$, and $B_3$, respectively. 
In contrast, the harmonic bars are shown in purple. 
Before time $t_8$, $z_1^1=z_1, z_2^1=z_2$ and $z_3^1=z_3$ serve as harmonic cycle representatives. 
At time $t_8$, $z_3$ dies as the triangle $t_8$ enters the filtration. 
And the addition of triangle $t_8$ causes $z_1$ and $z_2$ to have coboundary. 
A new cycle homologous to $z_1$ and harmonic at $t_8$ can be found by finding a solution to $\delta (z_1 + \partial x) =0$. 
This means $\delta \partial x = -\delta z_1 = -t_8$. 
Since $\delta \partial t_8 = 3t_8$, we can take $x=-\frac{1}{3} t_8$. 
The new harmonic cycle is then $z_1^2 = z_1 - \frac{1}{3}(\partial t_8)$. At time $t_9$, $z_1$ dies and clearly $z_1^2$ also dies. At time $t_8$, $z_2$ dies and similarly we get a new cycle $z_2^2 = z_2 - \frac{1}{3}(\partial t_8)$. This cycle dies at $t_9$ and a new cycle replacing it dies at $t_{10}$. 

In the right filtration, we again have cycles computed by the matrix reduction algorithm, from top to bottom, $\bar{z}_1 = t_1 - t_2 - t_3 +t_4$, $\bar{z}_2 = -t_1+t_2+t_5$ and $\bar{z}_3 = t_5 - t_6 + t_7$ serve as representatives for $\bar{B}_1, \bar{B}_1$, and $\bar{B}_3$, respectively. The harmonic bars are obtained using these basis elements in a similar fashion. At time $t_8$, the cycle $\bar{z}_1$ remains harmonic since it is not incident to $t_8$. 
As before, $\bar{z}_2$ becomes non-harmonic at $t_8$ and is replaced by a harmonic cycle that dies at $t_9$. 
The cycle $\bar{z}_3$ dies also at $t_8$. 

A matching provided by the stability of the persistence diagram needs to match $\bar{B}_2$ with $B_1$, and $\bar{B}_1$ with $B_2$. 
Now, even if $\bar{z}_1^1=\bar{z}_1$ dies immediate at $t_9$, its bar will have a surplus of length of at least $t_9 - t_8$ and this can be made arbitrarily large compared to $t_5-t_4$. 
Hence it cannot be matched to any bar on the left {\hcb} without incurring an arbitrary high cost to the matching.

==> sec-unstable-barcode.tex <==
\section{A First Attempt: Unstable Harmonic Chain Barcode}
\label{sec:unstable-barcode}

In this section, we discuss our first attempt at constructing a {\hcb} from a persistence barcode. 
Our approach is a natural one, however, we show that it does not lead to a stable barcode of harmonic chains. 
Nevertheless, our first attempt sheds light on how we might search for one that is stable, as discussed in~\cref{sec:stable-barcode}.

To avoid confusions, we use the following notations. 
Ordinary persistent homology gives rise to \emph{persistence barcodes}. 
An interval belonging to a persistence barcode is referred to as a \emph{persistence bar}. 
In our setting, we introduce \emph{\hcbs}. 
An interval belonging to a {\hcb} is called a \emph{harmonic bar}. 

\subsection{Constructing a Harmonic Chain Barcode from a Persistence Barcode}
\label{sec:first-attempt}

Starting from a persistence barcode, we assume there exists a choice of a homology class for each persistence bar, such that at each time $t$, the classes of existing bars at time $t$ form a basis of the homology group of $K_t$. There are many such choices, one such choice is represented by a function $\phi$ that maps persistence bars to homology classes as follows.
Let $B = [b, d)$ be a single interval (persistence bar) in the persistence barcode. 
$\phi$ maps each persistence bar $B$ to a chosen homology class, denoted by $\phi(B)$. The start of the interval $B$ is the birth of $\phi(B)$. 
Let $z_b$ be the harmonic cycle in the homology class $\phi(B)$. 
Starting from $b$, we follow through time until a time $s_1$ such that $\delta_{s_1}(z_b)\neq 0$. This implies that $\delta_{s_1}(z_b) = \sum \ell_j \sigma_j$, for some $\ell_j \in \Rspace$, where $\sigma_j$ are the simplices inserted at time $s_1$. 
At this point, the cycle $z_b$ dies entering $s_1$, and there is a bar $[b,s_1)$ in the {\hcb}. If $s_1 \neq d$, there has to be another cycle $z_1$ such that $[z_1] = [z_b]$ at time $s_1$, and $z_1$ is a cocycle in $K_{s_1}$. 
We therefore generate a new harmonic bar with a start time of $s_1$, and associate the cycle $z_1$ to it, and so on. After processing all (finite filtration) times, we obtain a {\hcb} subordinate to $\phi$. 

The above algorithm decomposes the persistence bars into a type of harmonic bars. The decomposition is guided by the choice of basis elements for each persistence bar by $\phi$. Each harmonic bar represents a unique harmonic cycle, hence, contains geometric information. 

\subsection{Example}

\cref{fig:first-attempt-example} presents an example where we compute the {\hcb} starting with the cycles for the persistence bars obtained with the standard matrix reduction algorithm for persistence homology; see~\cref{sec:unstable-barcode-details} for details in constructing such a {\hcb}.
The matrix reduction algorithm~\cite{edelsbrunner2010computational} to obtain persistence barcodes runs in the worst case $O(n^3)$, where $n$ is the number of simplices~\cite{Morozov2005}. 
We use the time stamps as the names of vertices and edges (from $1$ to $15$), and $t_i$ as the names of triangles ($t_1$ to $t_4$). 
We give simplices the standard orientation determined by the ordering of the vertices given by the insertion time. 
The procedure we describe in~\cref{sec:first-attempt} gives an algorithm that runs in $O(n^4)$ to extract a {\hcb} from the persistence barcode, since it makes a pass of the filtration in $O(n)$ time with a persistence barcode computed in $O(n^3)$ time. 

\begin{figure}[!ht]
    \centering
    \includegraphics[scale = 0.75]{first-attempt-example.pdf} 
    \caption{(a) A filtration of a simplicial complex, the time that a simplex is inserted is written next to the simplex. For the four triangles we have times $t_1 < t_2 < t_3 < t_4$. We also use these time stamps as  names of the simplices. (b) A part of the boundary matrix of the complex which is relevant to 1-dimensional homology. The boundary matrix is already reduced, therefore, the generators of persistent homology computed by the standard matrix reduction algorithm are given by columns of the matrix. (c) The 1-dimensional ordinary persistence barcode (in black). (d) The 1-dimensional {\hcb} (in purple) based on the cycles computed by the matrix reduction algorithm.}
    \label{fig:first-attempt-example}
\end{figure}

%------------
% Check 
%\delta(z_4^3) = 0
%= \delta(z_4) + 1/4 \delta(\partial t_1 + \partial t_2)
%= \delta(7+8-9) + 1/4 \delta(9+14-15 + 9+13-12)
%= 0 + 0 - (t_1 + t_2) + 1/4 (t_1 + t_2 + t_1 + t_1 + t_1 + t_2 + t_2 + t_2)
% = 0 
%------------

 

Although in this example, each harmonic chain becomes non-harmonic after the insertion of a simplex, this is not a general phenomenon. 
The harmonic bars can be longer than one time step.

\subsection{Instability}

In a {\hcb} subordinate to some choice of basis element $\phi$ constructed above, the harmonic bars can appear and disappear without much restrictions.
Therefore, it is expected that such {\hcbs}
are not stable. 
Here we demonstrate this instability by presenting an example that shows when the basis elements are given by the standard reduction algorithm of persistence homology, the resulting {\hcb} is not stable. In the example of Fig.~\ref{fig:instability}, we have two filtration that differ only by the ordering of insertion of edges at times $t_4$ and $t_5$. The filtration on the right has a bar that cannot be matched to the filtration on the left with low cost, namely $\bar{B}_1^1$. See~\cref{sec:unstable-barcode-details} for technical details of this example. 

\begin{figure}[!ht]
    \centering
    \includegraphics{instability.pdf}
    \caption{Changing the order of two simplices might introduce an arbitrary large change in the {\hcb}. The filtration differ by exchange of two edges appearing at $t_4$ and $t_5$. The ordinary persistence barcode is in black, whereas the {\hcb} is in purple (constructed using the basis given by the standard matrix reduction algorithm).}
    \label{fig:instability}
\end{figure} 
In summary, our first attempt at constructing {\hcbs} leads to unstable ones; more constraints need to be imposed to construct stable {\hcbs}, which is discussed in~\cref{sec:stable-barcode}.




==> socg-submission-donot-touch/sec-abstract.tex <==
The persistence diagram is a topological descriptor that plays a fundamental role in topological data analysis. 
Given a filtration of a topological space, a persistence diagram tracks the evolution of its homological features.
In this paper, we introduce a new class of diagrams, referred to as the harmonic persistence diagram, which tracks the evolution of geometric features in a filtration. 
A point in this diagram is uniquely associated with a single geometric feature, namely, a harmonic chain. 
A persistence diagram corresponds to many harmonic persistence diagrams, based on possible choices of harmonic chains. Thus the harmonic persistence diagrams are in general not stable. 
However, we show that there is a well-defined canonical harmonic diagram, directly obtainable from a filtration,  that is stable.  
Our work provides strong evidence in a growing list of literature that geometric (not just topological)  information can be recovered from a filtration and its persistence diagram. 




==> socg-submission-donot-touch/sec-background.tex <==
\section{Background}
\label{sec:background}

In this section, we present give the definitions of standard notions of (co)homology with real coefficients and harmonic chains. However, we explain more than needed for just recalling the algebraic definitions in order to draw an understanding that helps with the rest of the paper.

\subsection{Homology and Cohomology}
Let $K$ be a simplicial complex. We first give the standard orientation to the simplices of $K$. This means that we order the vertices of $K$ and assign to any simplex $\sigma$ the ordering of its vertices induced from ordering of all the vertices. This is also the ordering used in all our examples. From now on, we think of a simplex $\sigma$ to be supplied with the standard orientation. When we write simplices as an ordered set of vertices, for instance, $s=v_0v_1\cdots v_{i}$, then by convention $s=\sigma$ if the sign of the ordering $v_0v_1\cdots v_{i}$ agrees with the sign of the standard orientation, otherwise $s=-\sigma$.

For any integer $i$, the $i$-dimensional \textit{chain group} of $K$ with coefficients in $\Rspace$, denoted $C_i(K)$, is in fact an $\Rspace$-vector space generated by the set of $i$-dimensional (oriented) simplices of $K$. Let $K_i$ denote the set of $i$-simplices of $K$ and $n_i=|K_i|$. By fixing an ordering of the set $K_i$ we can identify any $i$-chain $c\in C_i(K)$ to an ordered $n_i$-tuple with real entries.
For each $i$, we fix an ordering once and for all for the $i$-simplices, and we therefore identify $C_i(K)$ and $\Rspace^{n_i}$. Note that the standard basis of $\Rspace^{n_i}$ corresponds under the identification to the basis of $C_i(K)$ given by the simplices with standard orientation.

The $i$-dimensional boundary matrix $\partial_i: C_i(K) \rightarrow C_{i-1}(K)$ is defined on a simplex basis element by the formula,

\[ \partial (v_0v_1 \cdots v_i)= \sum_{j=0}^{i} {(-1)^j (v_0\cdots v_{j-1}v_{j+1}\cdots v_i) }.\]

In the right hand side above, in the $j$-th term $v_j$ is dropped. The formula guarantees the crucial property of the boundary homomorphism: $\partial_{i} \partial_{i+1} = 0$. This simply means that the boundary of simplex has no boundary. The sequence $C_i(K)$ together with the maps $\partial_i$ define the \textit{simplicial chain complex} of $K$ with real coefficients, denoted $C(K)$. The group of $i$-dimensional \textit{cycles}, denoted $Z_i(K)$, is the kernel of $\partial_i$. The group of $i$-dimensional boundaries, denoted $B_i(K)$, is the image of $\partial_{i+1}$. The $i$-dimensional homology group of $K$, denoted $H_i(K)$, is the quotient group $Z_i(K)/B_i(K)$. As a set this quotient is formally defined as $\{ z+B_i(K); z\in Z_i(K)\}$. The operations are inherited from the chain group. In words, the homology group is obtained from $Z_i(K)$ by setting any two cycles which differ by a boundary to be equal. It is easily seen that all these groups are also $\Rspace$-vector spaces.

Consider the space $\Rspace^{n_i}$. The cycle group $Z_i(K) \subset C_i(K) = \Rspace^{n_i}$ is a subspace, that is, a hyperplane passing through the origin. Similarly, the boundary group $B_i(K)$ is a subspace, and is included in $Z_i(K)$. The homology group is the set of parallels of $B_i(K)$ inside $Z_i(K)$. Each such parallel hyperplane differs from $B_i(K)$ by a translation given by some cycle $z$. These parallels partition $Z_i(K)$. The homology group is then clearly isomorphic to the subspace perpendicular to $B_i(K)$ inside $Z_i(K)$. 

Simplicial cohomology with coefficients in $\Rspace$ is defined usually by the process of dualizing. This means that we replace an $i$-chain by a linear functional $C_i(K) \rightarrow \Rspace$, called an $i$-dimensional \textit{cochain}. The set of all such linear functions is a vector space isomorphic to $C_i(K)$ called the dual vector space, denoted $C^i(K)$ . For the purposes of defining harmonic chains, we must fix an isomorphism. We take the isomorphism that sends each standard basis element of $\Rspace^{n_i}$, corresponding to $\sigma$, to a functional which assigns 1 to $\sigma$ and 0 to other basis elements, denoted $\hat{\sigma} \in C^i(K)$. Any cochain $\gamma \in C^i(K)$ can be written as a linear combination of the $\hat{\sigma}$. Therefore, it is also a vector in $\Rspace^{n_i}$. The fixed isomorphism allows us to identify $C^i$ with $\Rspace^{n_i}$, and hence to $C_i$. Therefore, any vector $x \in \Rspace^{n_i}$ is at the same time a chain and a cochain.

The \textit{coboundary matrix} $\delta^i: C^i \rightarrow C^{i+1}$ is the transpose of $\partial_{i+1}$: $\delta^i = \partial_{i+1}^T$. It follows that $\delta_{i+1}\delta_i=0$, and we can form a \textit{cochain complex} $C^i$. The group of \textit{$i$-cocycles}, denoted $Z^i$ is the kernel of $\delta^i$. The group of \textit{$i$-coboundaries} is the image of $\delta_{i-1}$. The $i$-dimensional \textit{cohomology group}, denoted $H^i(K)$ is defined as $H^i(K) = Z^i(K)/B^i(K)$. All of these groups are again vector subspaces of $C^i(K)$ and thus of $\Rspace^{n_i}$.
It is standard fact that homology and cohomology groups with real coefficients are isomorphic.

The dimension of the $k$-dimensional homology group is called the $i$-th $\Rspace$-Betti number, denoted $\beta_i(K)$. 

\subsection{Harmonic Cycles} Recall that we identified chains with cochains. Therefore, we can talk about the coboundary of the cycles $Z_i(K)$. The \textit{harmonic $i$-cycles}, denoted $\har_i(K)$ is the group of those cycles which are also cocylces. Considered as subspaces of $\Rspace^{n_i}$, we have $\har_i(K) = Z^i(K) \cap Z_i(K)$.

\begin{lemma}[\cite{eckmann1944harmonische}]
    $\har_i(K)$ is isomorphic to $H_i(K)$. In other words, each homology class has a unique harmonic cycle in it.
\end{lemma}


\subsection{Persistent Homology}
Persistent homology tracks the change in homology over time or any 1-dimensional parameter. We start by a filtration of a simplicial complex $K$. A filtration assigns to each $r\in \Rspace$ a subcomplex $F_r \subset K$, in such a way that, if $r < s$, $F_r \subset F_s$. Since $K$ is finite, there is a finite set of values $t_1, \ldots, t_m \in \Rspace$ where the subcomplex $F_{t_i}$ changes. Setting $K_i = K_{t_i}$, $K_0 = \emptyset$, and writing $f_i:K_i \xrightarrow{} K_{i+1}$ for the inclusions, the filtration can be written as

\begin{equation}\label{eq:fcomplex}
    \emptyset = K_0 \xrightarrow{f_0} K_1 \xrightarrow{f_1} K_2 \xrightarrow{f_2} \cdots \xrightarrow{f_{m-2}} K_{m-1} \xrightarrow{f_{m-1}} K_m=K.
\end{equation}



Taking homology we obtain a sequence of homology groups and connecting homomorphisms (linear maps) called a \textit{persistence module}:

\begin{equation}\label{eq:fhomology}
 H_i(K_0) \xrightarrow{f_{0*}} H_i(K_1) \xrightarrow{f_{1*}} H(K_2) \xrightarrow{f_{2*}} \cdots \xrightarrow{f_{m-2*}} H(K_{m-1}) \xrightarrow{f_{m-1*}} H(K_m).   
\end{equation}

We denote the homology persistence module by $H(F)$. In general, a persistence module $M$ is defined as assigning to each $r\in \Rspace$ a vector space $M_r$, and for each pair $s<t$, a homomorphism $f_s^t: M_s \xrightarrow{} M_t$. For all $s<t<u$, the homomorphism are required to satisfy $f_t^uf_s^t= f_s^u$. In other words, $M$ is a functor from the poset $\Rspace$ seen as a category to the category of vector spaces. We try to avoid category theory language in this paper.


In this paper, we consider solely flirtations in which $K_i$ differs from $K_{i-1}$, $i=1,\ldots,m$, by exactly one simplex $\sigma_i$. Note that the boundary of the simplex has been added before the simplex.
A cycle $z \in Z_i(K)$ appears for the first time at some index $b \in \{t_0,\ldots,t_m\}$, where it creates a new homology class not previously existing. We say that the homology class is \textit{born} at $b$. Notice that at $b$ the dimension of the homology group increases by one. The homology class then lives for a while until it \textit{dies entering} $K_d$, when it lies in the kernel of the map induced on homology by the inclusion $K_b \subset K_d$. For $s\leq t$, let $f^{s,t}_i: H_i(K_s) \rightarrow H_i(K_t)$ denote the map induced on the $i$-dimensional homology by the inclusion $K_s \subset K_t$. The image of this homomorphisms, $f^{t,s}_i(H_i(K_t)) \subset H_i(K_t)$, is called the $i$-dimensional \textit{$(s,t)$-persistent homology group} denoted $H_i^{s,t}$. The group $H_i^{s,t}$, which in our case is also a vector space, consists of classes which exist in $K_s$ and survive until $K_t$. The dimensions of these vector spaces are the \textit{persistent Betti numbers}, denoted $\beta^{s,t}_i$.

%The $i$-dimensional homology classes that are born at $b$ and die entering $d$ are formally,

%$$\frac{f_{i}^{b,d} (Z_i(K_b))}{ f_{i}^{b-1,d} (Z_i(K_{b-1})) \oplus (B_i(K_b) \cap f_{i}^{b,d} (Z_i(K_b)))}.$$

%If we just compute the dimensions, we have the formula

%$$  .$$




An \textit{interval module}, denoted $I=I(b,d)$, is a persistent module of the form

\[ 0 \rightarrow \cdots \rightarrow 0 \rightarrow \Rspace \rightarrow \Rspace \rightarrow 0 \rightarrow \cdots \rightarrow 0.\]

In the above, $\Rspace$ is generated by a homology class and the maps connecting $\Rspace$'s map generator to generator. The first $\Rspace$ appears at index $b$ and the last
appears at $d$. The convention is that, for any $b \leq r < d$, $I_r = \Rspace$ and is $I_r=0$ for other $r$. Any persistence module can be decomposed into a collection of interval modules in a unique way \cite{}. Consequently, a homology class that lives in time period $(b,d)$ can be written as a linear combination of intervals.
Each interval module is determined by the index of the first $\Rspace$, or the time it is born and the index of the last $\Rspace$ where it dies, which can be $\infty$.
The collection of $(b,d)$ for all interval modules is called the \textit{persistent homology barcode}. When plotted as points in a plane the result is the \textit{persistence diagram}. The persistence diagram therefore contains a summary of the homological changes in the filtration. 

==> socg-submission-donot-touch/sec-harmonic-diagrams.tex <==
\section{The Harmonic Persistence Diagrams}
\label{sec:harmonic-diagrams}

Consider a filtration $F$ and a homology class $h\in H(K_b)$ born at time $b$ which dies entering $K_d$. The dimension of homology increases at time $b$. The class $h$ contains a unique harmonic cycle $z_b$. We say that the harmonic cycle $z_b$ is \textit{born} at time $b$. When a persistent homology class dies (i.e., becomes a boundary), then clearly the corresponding harmonic cycle also \textit{dies}. Contrary to the ordinary persistent homology, these are not the only situations where a harmonic cycle is born, or dies. In brief, a harmonic cycle dies whenever it is not a cocycle anymore. It is easily seen that, when a cycle is no more a cocylce, it can never become a cocylce in the future. When a harmonic cycle dies a new harmonic cycle is born in the same homology class. In this sense, the harmonic barcode and diagram are refinements of the ordinary persistence barcode and diagram.   

We now give a formal definition. We first choose a basis for persistent homology. Each scheme for choosing a basis defines a type of harmonic diagram.

Consider the persistence module of homology groups $H(F)$. Recall that $H(F)$ can be written uniquely as a summation of interval modules,

\[ H(F) \cong \bigoplus_{j} I(b_j,d_j).\]

Let $B = \{(b_j,d_j)\}$ be the collection of intervals, $b_i,d_i \in \Rspace \cup \{+\infty\}$. We fix an isomorphism $\phi = \{\phi_t\}$ realizing the above relation, which amounts to choosing a basis element for each interval. More formally, let $\phi_t: B \rightarrow H(K_t)$ be functions such that,
\begin{enumerate}
    \item $\phi_t$ maps intervals $(b_i,d_i)$ such that $b_i \leq  t < d_i$ injectively to a collection of basis elements in $H(K_t)$, and other intervals to 0,

    \item The non-zero images of the same interval under different $\phi_t$, are mapped to each other by the homomorphisms $f^*_i$.
\end{enumerate}

A choice of basis satisfying these two conditions is, for instance, provided by the persistence reduction algorithm~\cite{edelsbrunner2002topological,zomorodian2005topology} used to compute the ordinary persistence barcode.

Next, we define a new persistence module $\Gamma = \Gamma(\phi)$ as follows. For all $r\in \Rspace$, we set $\Gamma_r = H(F_r)$. For any $s<t$, we define new homomorphisms $g_s^t: H(K_{s}) \rightarrow H (K_{t})$, by defining their value on the basis elements $\phi_t(B)$. Let $h \in H(K_{t})$ be a non-zero homology class in the image of $\phi_t$. There is a unique cycle $z \in h$ which is also a cocycle.  We set $g_s^t(h) = f_{s*}^t(h)$ if $z$ is a cocycle in $K_{t}$, and, $g_s^t(h) = 0$ otherwise. We call $\Gamma$ the \textit{harmonic filtration subordinate to $\phi$}. This is a persistence module. 

It follows from the decomposition theorem for persistence modules~\cite{crawley2015decomposition} that the filtration $\Gamma$ can be written as a linear combination of basis interval modules. Each interval module has birth and a death time. We call the collection of these intervals the \textit{harmonic persistence barcode subordinate to $\phi$}, and we call 
the corresponding diagram, the \textit{harmonic persistence diagram subordinate to $\phi$}. 

Observe that each harmonic interval, by definition of the $g_s^t$, corresponds to a unique harmonic cycle. The harmonic persistence barcode and diagram therefore track features which have a very well-defined and unique geometric entity associated with them. 


We now present a more intuitive definition of harmonic persistence barcode. We start from the persistence barcode. Let $B = (b,d)$ be a single bar in the persistence barcode. The start of the interval is birth of a homology class and an increase in dimension of homology. We take the basis element given by $\phi$ for the barcode. Let $z_b$ be the harmonic cocycle in that homology class. We follow through time until a time $s_1$ where there is a simplex $\sigma$ added to the complex such that it is incident to (simplices with non-zero coefficient in) $z_b$ and such that $\delta_{s_1}(z_b) = \ell \sigma \neq 0$, for some $\ell \in \Rspace$. Here the subscript $s_1$ shows we are considering the coboundary in $K_{s_1}$. 
At this point, the cycle $z_b$ dies entering $s_1$, and there is a bar $(b,s_1)$ in the harmonic barcode. If $s_1 \neq d$, there has to be another cycle $z_1$ such that $[z_1] = [z_b]$ and $z_1$ is a cocycle in $K_{s_1}$. We generate a new harmonic bar with start time $s_1$. After processing all times $t_i$, we obtain the harmonic persistence barcode subordinate to $\phi$. 
This process decomposes the persistence intervals into harmonic intervals. The decomposition is guided by the choice of basis elements for each bar by $\phi$. Each harmonic interval represents a unique harmonic cycle, hence, contains geometric information.

\subsection{Example}

Figure~\ref{fig:harmonicexample} presents an example where we have computed the harmonic persistent barcode starting by the cycles for the bars computed by the standard reduction algorithm. 
We use the time stamps as the names of the simplices. Also we give simplices the standard orientation determined by the ordering of the vertices given by the insertion time. The procedure we describe gives an algorithm of running time $O(n^4)$ where $n$ is the number of simplices.


Let $B_1=[9,t_4]$ be the longest bar in the persistence diagram, it is represented by the cycle $z_1 = 7+8-9$. Let $B_2 = [11, t_3]$ be the next longest bar, $z_2 = -11 +10 +9$.  Let $B_3 = [13,t_2]$ be the next bar, it is represented by $z_3=13-12+9$. Finally, let $B_4 = [15,t_1]$ be the last bar, it is represented by $z_4=15-14+9$.

To obtain harmonic bars we sweep from left to write. At time $t_1$, all of the basis cycles $z_i$ get a coboundary. From these, the homology class of $z_4$ becomes trivial, and others are still non-trivial. For instance, if we take $z_1$, its homology class is still non-trivial. We can find a new harmonic cycle in its class by finding $x$ such that $\delta(z_1 + \partial x) =0$ at time $t_1$. This implies $-t_1 = \delta(z_1) = - \delta \partial x$. Since $\delta \partial t_1 = 3 t_1$, we can set $x = 1/3 t_1$, and the new harmonic chain is $z^1_1 = z_1 + 1/3 \partial (t_1)$. We get similarly $z^1_2 = z_2 - 1/3 \partial (t_1)$ and $z^1_3 = z_3 - 1/3 \partial (t_1)$. At time $t_2$, $z_3$ and hence $z^1_3$ die. Cycle, $z^1_1$ gets a coboundary $- t_2$ and $\delta t_1$ gets a coboundary $t_2$ hence $\delta_{t_2} (z^1_1) = -2/3 t_2$. A new harmonic cycle is $z_1^2 = z_1 + 1/4(\partial t_1 + \partial t_2)$. Similarly, $z^2_2 = z_2 - 1/4(\partial t_1 + \partial t_2)$. At time $t_3$, the cycle $z_2$ and its harmonic homologous cycles die. $z_1^2$ also becomes non-harmonic and will be replaced by another harmonic cycle that will die at $t_4$. 

We note that although each harmonic chain becomes non-harmonic after insertion of a simplex in this example, this is not a general phenomenon. The harmonic bars can be long.


\begin{figure}
    \centering
    \includegraphics[scale = 0.75]{harmonicexample.eps} 
    \caption{a) A filtration of a simplicial complex, the time that a simplex is inserted is written next to the simplex. For the four triangles we have times $t_1 < t_2 < t_3 < t_4$. We also use these time stamps as the name of the simplex. b) Part of the boundary matrix of the complex which is relevant to 1-dimensional homology. The boundary matrix is already reduced, therefore, the generators of persistent homology computed by the standard reduction algorithm are given by columns of the matrix. c) The ordinary persistence barcode. d) The harmonic barcode based on the cycles computed by the standard reduction algorithm.}
    \label{fig:harmonicexample}
\end{figure}

\subsection{Instability}
Due to the fact that in a harmonic diagram subordinate to some choice of basis element $\phi$ the bars can appear and disappear without much restrictions, it is expected that such diagrams
are not stable. Here we demonstrate this by presenting an example that shows when the basis elements are given by the standard reduction algorithm of persistence homology the resulting harmonic barcode and diagram are not stable. 

Figure~\ref{fig:instability} shows two filtrations whose only difference is the exchange of times when edges $12$ and $23$ are inserted. We use $t_i$ to label simplices other than vertices which are labeled 1 to 4. The middle barcode is the persistent barcode. In the left filtration the standard algorithm gives the following cycles for the bars, from top to bottom, $z_1 = -t_1+t_2+t_4$, $z_2 = -t_3+t_4+t_5$ and $z_3=t_4-t_6+t_7$. The bottom bars are harmonic bars. At time $t_8$, $z_3$ dies. However, addition of triangle $t_8$ causes $z_1$ and $z_2$ to have coboundary. A cycle homologous to $z_1$ and harmonic at $t_8$ can be found by finding a solution to $\delta (z_1 + \partial x) =0$. This means $\delta \partial x = -\delta z_1 = -t_8$. Since $\delta \partial t_8 = 3t_8$, we can take $x=-1/3 t_8$. The new harmonic cycle is then $z^1_1 = z_1 - 1/3(\partial t_8)$. At time $t_9$, $z_1$ dies and clearly $z^1_1$ also dies. At time $t_8$, also $z_2$ dies and similarly we get a new cycle $z^1_2 = z_2 - 1/3(\partial t_8)$. This cycle dies at $t_9$ and a new cycle replace it which dies at $t_{10}$. 

We now consider the filtration at the right in Figure~\ref{fig:instability}. We now have cycles computed by the standard algorithm, from top to bottom, $z_1 = t_1 - t_2 - t_3 +t_4$, $z_2 = -t_1+t_2+t_5$ and $z_3 = t_5 - t_6 + t_7$. Note that how a matching provided by the stability of the persistence diagram needs to  match the middle bar of right filtration with the top bar of the filtration of left, and the top bar of the right to the middle bar of the left. At time $t_8$, the cycle $z_1$ will remain harmonic since it is not incident to $t_8$. As before, $z_2$ becomes non-harmonic at $t_8$ and will be replaced by a harmonic cycle that dies at $t_9$. Cycle $z_3$ dies also at $t_8$. Now even if $z_1$ dies at the immediate next time, which is, $t_9$, its bar will have a surplus of length of at least $t_9 - t_8$ and this is arbitrarily large compared to $t_5-t_4$. Hence it cannot be matched to any bar on the left harmonic barcode without incurring an arbitrary high cost to the matching.



\begin{figure}
    \centering
    \includegraphics{instability.eps}
    \caption{Changing the order of two simplices might effect an arbitrary large change in the harmonic barcode. The filtration differ by exchange of two edges. The middle bars (black) are the ordinary persistence barcode, the bottom bars (purple) are harmonic diagrams using the basis given by the standard reduction algorithm.}
    \label{fig:instability}
\end{figure}


==> socg-submission-donot-touch/sec-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

There are two primary tasks in topological data analysis (TDA)~\cite{dey2022computational,edelsbrunner2010computational,zomorodian2005topology}: reconstruction and inference. 
In a typical TDA pipeline, the data is given as a point cloud in $\Rspace^m$.  
A "geometric shape" $K$ in $\Rspace^m$ is constructed from the point cloud, usually as a simplicial complex, and $K$ is taken to represent the (unknown) space $X$ from which the data is sampled. 
$X$ is then studied using $K$ for properties that are invariant under invertible mappings (technically, homeomorphisms). 
The deduced "topological shape" is not specific to the complex $K$ or the space $X$, but is a feature of the homeomorphism type of $K$ or $X$. 
For example, a standard round circle has the same topological shape as any closed loop such as a knot in the Euclidean space. 
Although topological properties of $X$ alone are not  sufficient to reconstruct $X$ exactly, they are among a few global features of $X$ that can be inferred from the data sampled from $X$. 

A persistence diagram~\cite{Chazal, cohen2005stability, edelsbrunner2002topological} (or equivalently, a persistence barcode~\cite{CarlssonZomorodianCollins2004,Ghrist2008}) captures the evolution of homological features in a filtration constructed from a simplicial complex $K$. 
It is a multiset of points in the extended plane, where a point in the persistence diagram encodes the birth and death time of a homological feature in the filtration. 
Equivalently, a persistence barcode consists of a multiset of intervals in the extended real line, where the start and end point of an interval (i.e.,~a bar) map to the birth and death time of a homological feature. 
A main drawback of homological features is that they ignore the geometric information in $K$, even though they are defined on a set of simplicial chains with  distinct geometric features. 
In this paper, we aim to recover geometric information from a filtration and its persistence diagram. 
We introduce a new class of diagrams, referred to as the \emph{harmonic persistence diagram}, which tracks the evolution of geometric features in a filtration. 
A point in this diagram is uniquely associated with a single geometric feature, namely, a harmonic chain, and tracks its birth and death in a filtration.  
 
A persistence diagram is stable, and this stability is crucial for data science applications. 
The stability means that small changes in the data imply only small changes in the diagram. 
It turns out that a persistence diagram corresponds to many harmonic persistence diagrams, based on possible choices of harmonic chains. Therefore, a harmonic persistence diagram is, in general, not stable.  
However, we show that there is a well-defined canonical harmonic diagram that is stable.

Defining a canonical harmonic diagram that is stable  requires some care. To do so, we start by reviewing the \emph{Elder Rule} in the computation of a persistence diagram, that is, an older homology class persists if it merges with a younger homology class in the filtration. 
Imagine that we are tracking the homology of a filtration of $K$ (with real coefficients $\Rspace$), constructed by adding simplices, one at a time.
At the filtration time $t$, we have maintained a set of homology \emph{basis}, that is, a maximal linearly independent set of homology cycles (of each dimension). 
Then a simplex $\sigma$ is added at time $t+1$ that destroys a homology class, thus reducing the dimension of a homology group. 
At time $t+1$, a linear combination $\tau$ of our basis elements is homologous to the boundary of the added simplex $\sigma$, and hence a homology class is destroyed. 
The Elder Rule says that at time $t+1$, we destroy the youngest of the basis elements that appear in $\tau$.
At the same time, other homology classes persist in the filtration, although we might need to change the basis elements that represent these homology classes at time $t+1$.  

Now, is it possible to assign specific cycles (representatives) to a point in the persistence diagram?  
Such an assignment is desirable, since then each point would correspond to a unique geometric feature. 
There are two choice levels: first, we choose a basis for persistent homology in a consistent way; and second, we choose a cycle inside a basis element. 
Both levels of choices involve choosing from among distinct geometric features of data.  

In this paper, we work with harmonic cycles, which  immediately remove the second level of choices in a natural way, since there is always a unique harmonic cycle in a homology class. 
However, in general, the harmonic cycles appear and disappear at times where the dimension of homology groups do not change. 
Consequently, our harmonic persistence diagram is, in general, a refinement of a persistence diagram. 
In a nutshell, for any choice of basis for persistent homology, we refine the persistent diagram so that each point can be represented by a unique harmonic chain. 
A harmonic persistence diagrams defined in this manner, although interpretable, is not stable, and we present examples of such instability.

Finally, we define what we call a canonical harmonic persistence diagram. 
Unlike a persistence diagram, our canonical harmonic diagram is defined using a global analysis of the filtration (w.r.t. time). 
We show that such a diagram can be constructed in polynomial time and is stable.
%The extra conditions required for stability are satisfied in common settings where stability is proved for ordinary persistent diagram.

==> socg-submission-donot-touch/sec-related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Harmonic chains were first studied in the context of functions on graphs. 
They were identified as the kernel of Laplacian operators on graphs~\cite{Kirchhoff}. 
The graph Laplacian and its kernel are important tools in studying graph properties, see~\cite{MERRIS1994143,mohar1991laplacian} for surveys. 
Eckmann~\cite{eckmann1944harmonische} introduced the higher-order Laplacian for simplicial complexes, and proved the isomorphism of harmonic chains and homology. 
Horak and Jost~\cite{horak2013} defined the weighted Laplacian for simplicial complexes. 
Already the theoretical results on Laplacian~\cite{horak2013} anticipated the possibility of applications, as the harmonic chains are thought to contain important geometric information.
This has been validated by recent results that use curves of eigenvalues of Laplacians in a filtration in data analysis~\cite{chen2022, wang2020persistent}. The persistent Laplacian~\cite{memoli2022persistent} and its stability~\cite{liu2023algebraic} is an active research area. The Laplacian also has been applied to improve the mapper algorithm~\cite{mike2019}, and for coarsening triangular meshes~\cite{keros2023spectral}. The stability of higher-order Laplacians in a simplicial complex is studied in~\cite{guglielmi2023quantifying}. Due to the intimate relationship of harmonic chains and Laplacians, harmonic chains could find applications in areas that Laplacians have been used.


Computing reasonable representative cycles for persistent homology is also an active area of research. 
Here, usually an optimality criterion is imposed on cycles in a homology class to obtain a unique representative. 
For a single homology class,~\cite{chen2011hardness, Dey2010-1, chambers2022complexity} consider different criterion for optimality of cycles. For persistent homology, Dey et al.~\cite{dey2020computing} studied the hardness of choosing optimal cycles for persistence bars. 
Volume-optimal cycles have been computed for persistent homology~\cite{Obayashi}. The harmonic chains have been used as representative of homology classes for studying the brain~\cite{lee2019}.

The most relevant paper to ours is the work of Basu and Cox~\cite{basu2022harmonic}. 
In fact, the term "harmonic persistent diagram" appears also in~\cite{basu2022harmonic}\footnote{We were unaware of this paper when coming up with the same name.}. They also have the same goal as we do, namely, to associate geometric information to each point in a persistence diagram in order to obtain a more interpretable data feature. 
They associate a subspace of harmonic chains to each point in the (ordinary) persistence diagram. Then, they prove stability for their harmonic diagrams, by considering subspaces as points of a Grassmannian manifold and measuring distances in the Grassmannian. To the best of our knowledge, we are the first to consider different diagrams than persistent homology diagram with to goal of achieving a more geometric stability, either by subdividing the bars, or defining new bars based on certain types of cycles. 

Authors of~\cite{de2021parallel} use harmonic cycles in a persistent homology setting to compute the persistence diagram.  A. Lieutier~\cite{Lieutier} studies the harmonic chains in persistent homology classes.

==> socg-submission-donot-touch/sec-stable-diagrams.tex <==
\section{Stable Harmonic Diagrams}
\label{sec:stable-diagrams}

As we have seen in the above, a harmonic diagram resulting from choosing harmonic cycles for each bar in the persistence barcode is not stable. In this section, we present a harmonic persistence diagram which is stable. 
We focus on a fixed dimension $d$. Let the set of bars of the barcode of dimension $d$ be denoted by $\mathcal{B} = \mathcal{B}(d) = \{(b_i, d_i), i=1, \ldots, m_d \}$. 

%Recall that, given a filtration of complexes and its persistence barcode, we process the bars from left to right, or from the smallest birth time
%to the largest birth time. 

%Since we are assuming that at each time we add only a single simplex, the very first $d$-cycle generated in the filtration must always be a harmonic cycle, as there is no other cycle
%in the homology class. Hence, there is no choice for the harmonic cycle of the first bar. Let $t$ be the time or the sweep parameter.


Recall that the space of harmonic $d$-cycles at time $t$, which we denote $\har_d(K_t)$, is isomorphic with the $d$-homology $H_d(K_t)$. A cycle might be a harmonic cycle when it is first created,
and then it might seize being harmonic at a later time (i.e., get a non-zero coboundary), or it might become a boundary, or might be harmonic up to infinity.

\begin{definition}
 For $z \in Z(K)$, let the \emph{harmonic span of} $z$, denoted $span(z)$, be the interval (open from the right) in the filtration during which $z$ is a harmonic (non-trivial) cycle. If a cycle is non-harmonic at birth its span has length $0$. If a cycle is harmonic in $K$ its span has length $\infty$. We denote the length of the span of $z$ by $|span(z)|$.   
\end{definition}


\begin{definition}
 Let $ \Gamma \subset Z(K)$ be a subspace of cycles. Observe that $\Gamma$ is filtered by the filtration of $Z(K)$. Let $\rho_1$ be the maximum span-length of any harmonic cycle in $\Gamma$, let $z_1 \in \Gamma$ be a cycle with span-length $\rho_1$. Define now $z_i$ inductively by taking
it to be \textbf{a} cycle which i) is independent of the set $\{z_j\}$ (as elements of $\Gamma$), $j<i$, and, ii) among all cycles satisfying i) maximizes the harmonic span-length. Let $\rho_i = |span(z_i)|$.
We call the sequence $\rho_1 \geq \rho_2 \geq \cdots $ the \emph{maximum span-length sequence} for $\Gamma$. We call the sequence $z_1, z_2, \ldots$ a sequence of cycles
\emph{realizing the maximum span-length sequence}.

The \emph{canonical harmonic persistence diagram (or barcode)} of a filtration $F$, denoted $\chd(F)$, is the set of spans of cycles realizing a maximum span sequence for $Z(K)$.

\end{definition} 

In other words, the maximum span-length sequence is lexicographically largest sequence of span-lengths defined by independent cycles.
We need to argue that the canonical harmonic diagram is independent of the choices made in the above definition. We also need to prescribe a method to compute the bars. 
For these purposes, we compute the canonical harmonic diagram by sweeping time from $-\infty$ to $\infty$. At any time $t$, we maintain a set of cycles $R(t)$ satisfying the invariant that,%For these purposes, we obtain the same set of bars by a different process where we sweep the parameter $t$ from $-\infty$ to $\infty$, and we maintain a set of cycles $R(t)$ satisfying the invariant that, at any time $t$,

\begin{itemize}
    \item the set $R(t)$ contains cycles realizing a maximum span sequence for $Z(K_t) \subset Z(K)$.
\end{itemize}


%That is to say, $R(t)$ contains cycles from $K_t$, and those representatives are still harmonic at $t$. $R(t)$ is then
%a basis for $\har_d(K_t)$. The set of spans defined by the cycles in the union of $R(t)$ can be taken as a second definition 
%of a canonical harmonic diagram.

The following Lemma describes the change from $R(t_i)$ to $R(t_{i+1})$, it also implies that different choices in the definition do not provide different diagrams.


\begin{lemma}\label{l:greedy}
    Assume that the harmonic representatives $R(t_{i})$ satisfy the invariant at time $t_i$. Then, at time $t_{i+1}$, if the dimension of the harmonic chains increases, to obtain $R(t_{i+1})$ satisfying the invariant, it is enough to add to $R(t_{i})$ the longest span belonging to cycles born at $t_i$.

    %\begin{enumerate}
    %    \item if the dimension of the harmonic chains increases, to obtain $R(t_{i+1})$ satisfying the invariant, it is enough to add to $R(t_{i})$ the longest span belonging to cycles born at $t_i$,

    %    \item if the dimension of the harmonic chains decreases, then exactly one span in $R(t_{i})$ ends at $t_{i+1}$ and, to obtain $R(t_{i+1})$ satisfying the invariant, it is enough to remove that cycle to obtain $R(t_{i+1})$,

    %    \item if the dimension of harmonic cycles is unchanged, we can set $R(t_{i+1})=R(t_{i})$.
    %\end{enumerate}
    
\end{lemma}

\begin{proof}
    Let $\sigma$ be the simplex inserted at time $t_{i+1}$. If $\sigma$ is not $d$ or $d+1$ dimensional then the set of $d$-cycles and harmonic $d$-cycles do not change. We then can set $R(t_{i+1})=R(t_{i})$.

    Suppose $\sigma$ is $d$-dimensional. Then it might create new harmonic cycles. If this does not happen we can set $R(t_{i+1})=R(t_{i})$. Note that a new harmonic cycle is created if and only if a new $d$-homology class is born. In this case, the dimension of harmonic cycles increases. Note that $\har (K_{t_{i}}) \subset \har (K_{t_{i+1}})$ is a subspace of codimension 1.
    
    Let $N$ be the maximum death time of all harmonic cycles generated at time $t_{i+1}$. Note that $N-t_{i+1}$ is the maximum span length of these cycles and their span is determined by their death time. Let $\zeta \in \har (K_{t_{i+1}})$ be a cycle that realizes the span $[t_{i+1},N)$. Set $R' = R(t_i) \cup \{ \zeta \}$. We claim that $R'$ satisfies the invariant at time $t_{i+1}$. %It is evident that $R'$ is a basis of $\har (K_{t_{i+1}})$. 

    To prove the claim we consider how the maximum span-length sequence of $Z(K_{t_{i+1}})$, denoted, $\rho_1 \geq \rho_2 \geq \cdots $ is constructed. Recall that we first take a cycle with maximum span length. If this cycle is in $Z(K_{t_{i}})$ then this span length will appear as span interval with maximum length in $R(t_i) \subset R'$ by the induction hypothesis. This will be again true for the second number, etc. Let $\rho_j$ be the first appearance of a number that is not in the maximum span-length sequence for $Z(K_{t_{i}})$ (note that it can be that $\rho_j = \rho_{j-1}$, in this case $\rho_j$ is one more repetition of the same number). A realizing cycle is in $Z(K_{t_{i+1}}) - Z(K_{t_{i}})$ and it has to have the maximum span length in this set. Therefore, $\rho_j = N$ and $\zeta$ realizes this span-length. Now we claim that the rest of the cycles in a sequence realizing the maximum span-length sequence for $Z(K_{t_{i+1}})$ must come from $Z(K_{t_{i}})$ and hence their span-lengths must appear among spans of $R(t_i) \subset R'$.

    To prove the claim let's assume for the sake of contradiction that a second cycle appearing in order of span-lengths $\zeta' \in Z(K_{t_{i+1}}) - Z(K_{t_{i}})$ has a span-length in the sequence, and $|span(\zeta')|\leq |span(\zeta)|$. $\zeta'$ must have a non-zero coefficient for $\sigma$ say $\beta$. Let $\alpha \neq 0$ be the coefficient of $\sigma$ in $\zeta$. We can form the cycle $\chi = \alpha/ \beta \zeta' - \zeta \in Z(K_{t_{i}})$. When $\chi$ becomes non-harmonic, i.e., at the first $t$ such that $\delta_t(\chi)\neq 0$, at least one of $\zeta'$ and $\zeta$ must also become non-harmonic. Since the death time of $\zeta$ is equal or larger than $\zeta'$, the death time of $\chi$ is at least that of $\zeta'$. Since $\chi$ already exists at time $t_{i}$ it must be that $|span(\chi)| > |span(\zeta')|$. This contradicts the selection of $\zeta'$ as it is in a space generated by cycles of larger span-length $\zeta$ and $\chi$. This finishes the argument.

    If $\sigma$ is $d+1$-dimensional, the set of $d$-cycles $Z(K_t)$ does not change and we can set $R(t_{i+1}) = R({t_i})$.

    
    
\end{proof}



\begin{corollary}
The number of bars in the canonical harmonic barcode equals the number of bars in the persistent homology barcode.
\end{corollary}

\begin{proof}
By the Lemma, a new bar is added if and ony if the dimension of $d$-homology increases.
\end{proof}


\begin{corollary}
    There is an algorithm for computing a the canonical harmonic persistence diagram that runs in $O(n^4)$ time, where $n$ is the number of simplices in $K$.
\end{corollary}

\begin{proof}
At each insertion of a simplex, say $d$-dimensional at time $t_i$ where the dimension of $d$-cycles increases, we compute for all times $t_j > t_i$, the subspaces (of $Z(K)$) $A_{ij} = Z(K_{t_i}) \cap \har(K_{t_j})$, and then take the largest time $t_j$ where $A_{i,j} - Z(K_t) \neq \emptyset$. These operations can be done in $O(n^3)$ per time step and $O(n^4)$ in total.
\end{proof}

The following lemma is also very useful.

\begin{lemma}
The spans of non-zero, finite length in the canonical harmonic diagram die at distinct times.
\end{lemma}

\begin{proof}

Suppose $\sigma$ is $d+1$-dimensional which is inserted at time $t_{i+1}$. $\sigma$ can kill a $d$-homology class or makes a harmonic chain non-harmonic. If it makes a harmonic chain non-harmonic, insertion of $\sigma$ reduces the dimension of harmonic $d$-cycles. Therefore this can happen only if $d$-kills a $d$-homology class. Assume this is the case. Let $z_0$ be the cycle for a bar in the harmonic diagram whose whose coboundary is non-zero at $t_{i+1}$, that is, span of $z_0$ ends at $t_{i+1}$, and we choose $z_0$ such that the span-length of $z_0$ is minimum. Observe that, there must be at least one such cycle in $R(t_i)$ since otherwise we will have at time $t_{i+1}$ the same dimension of harmonic chains as time $t_i$. Moreover, note that since independent cycles representatives of bars are created at distinct times (by Lemma~\ref{l:greedy}), there is a single span whose length is minimum and ends at $t_{i+1}$. 

Crucially, we need to argue that no other span ends at $t_{i+1}$ so that other representatives in $R(t_i)$ remain harmonic at time $t_{i+1}$. To see this, assume $z_1 \neq z_0 \in R(t_i)$ is the next shortest span that ends at $t_{i+1}$. Then it should be that $\delta_{i+1} (z_1) = \alpha \sigma$ for some $\alpha \neq 0$, and similarly, $\delta_{i+1}(z_0) = \beta \sigma$ for some $\beta \neq 0$. Again, using $z_0$ and $z_1$ we can find a new chain $y = \alpha /\beta z_0 - z_1$ in the subspace generated by $z_0$ and $z_1$ which survives $t_{i+1}$. The birth time of this cycle is at most the birth time of $z_0$ (since $z_1$ is born before $z_0$, span of $z_1$ being longer), and it survives $t_{i+1}$. Thus its span length is longer than that of $z_0$. Replacing $z_0$ with $y$ we obtain a new set of cycles generating $Z(K_{t_i})$. Note that $z_0$ is the shortest span among all spans of $Z(K_{t_i})$ which include $t_i$. The corresponding span length sequence is an improvement of the sequence of $R(t_i)$. This contradicts the invariant for $R(t_i)$. 





    
    %Either a representative in $R(t_i)$ becomes a boundary or it becomes equal to a combination of other representatives. In first case, the representatives of $R(t_i)$ involved has already the smallest span in any sequence realizing the maximum spans sequence. In the second case, a combination $c$ of harmonic cycles would satisfy $\delta(c)\neq 0$. In this case, at least one of the chosen representative elements $r \in R(t_i)$ has to satisfy $\delta(r)\neq 0$.
    %This will be the representative with smallest span.   
    %Therefore, we need only drop the representative with smallest span in both cases. If there are multiple representatives with smallest span, we drop one whose coboundary assigns a non-zero value to $\sigma$. The remaining representatives still satisfy the invariant.
    %\Salman{We should say that, by the first part, there is at most $d+2$, $d$-dimensional harmonic cycles containing $d$-simplices of $\sigma$. We need to replace each one $z$ by $z+x\delta \sigma$.}

    
\end{proof}


\subsection{Example}
Figure~\ref{fig:charmonicexample} depicts the canonical persistent diagram of the example in Figure~\ref{fig:harmonicexample}. At time $9$ the first cycle $r_1 = 7+8-9$ is created. This will create a bar that will end at $t_1$ when the cycle $r_1$ gets a coboundary. At time $11$ a new dimension in cycle space is added. To compute a cycle that survives most, we can start from $t=+\infty$ and compute the largest $t$ such that $Z(K_{11}) \cap \har(K_t) = Z(K_{11}) \cap \ker (\delta_t) \neq \{ 0 \}$. By Lemma~\ref{l:greedy}, this will be the only change necessary in our representatives. take the cycle $r_2 = 7+8+10-11$. $r_2$ is harmonic, and it survives up until $t_3$. One can check that if a cycle has non-zero coefficient for $9$ it has to die earlier, and therefore, $r_2$ represents the longest bar generated at $11$, namely, $[11,t_3]$. At time $13$, with a logic similar to time $11$, we obtain the cycle $r_3$ which defines a bar $[13,t_2]$. Now at time $15$, we have all possible edges so there has to be a harmonic chain that survives up to $t_4$. We take $r_4 = 3r_1 - \partial( t_1+t_2+t_3)$. One checks easily that $\delta_t \partial (r_j) = \delta_t(9)$, for $j=2,3,4$. Therefore, $\delta_t(r_4) = 3\delta_t(9)-3\delta_t(9)=0$ for $ 15 \leq t < t_4$. 

\begin{figure}
    \centering
    \includegraphics[scale=.85]{charmonicexample.eps}
    \caption{The canonical harmonic barcode for the complex in Figure~\ref{fig:harmonicexample}.}
    \label{fig:charmonicexample}
\end{figure}


\subsection{Stability}
We express the stability of the harmonic persistence diagram by considering the typical setting of when two simplices exchange their order of insertion into the filtration. We then
consider the general case where there is an $\eps$-interleaving between the two filtrations $F_1$ and $F_2$. In this case, we stop short of proving the analogous stability, however, we 
can prove that the maximum span-length sequence is stable, given further natural conditions on the interleaving.

\begin{theorem}
Let the filtrations $F$ and $F'$ be related by exchange of the order of insertion of two simplices $\sigma_1$ and $\sigma_2$. Assume before and after the exchange simplices are inserted at times $t_1$ and $t_2$, with $|t_2-t_1|=\eps$. Then the bottleneck distance between the canonical harmonic persistence diagrams satisfies,
\[ d_B( \chd(F), \chd(G) ) \leq  \eps \]

\end{theorem}
\begin{proof}
In brief, each span changes by $\eps$ from at most one side, and the order of lengths do not change. In more detail,
if both simplices are $d$-dimensional, then the birth time of two consecutive spans in the maximum sequence are exchanged. The spans after this change,
are still a maximum span sequence, since the lengths differ by a more than $\eps$ from the endpoints. We can match the span that end at the same time from each diagram together, see figure~\ref{fig:stableexample}. An analogous argument works for the case where the two simplices exchanged are $d+1$-dimensional. If one simplex is $d$ and the other is $d+1$-dimensional, and also in other cases, the birth and death time of two distinct spans move by $\epsilon$ and these will be matched to their original spans.

\end{proof}

Using standard theory~\cite{edelsbrunner2010computational}[Chapter VIII] we get the bottleneck stability for sub-level-set filtrations.

\begin{theorem}
Let $K$ be a simplicial complex and $f,g: K \xrightarrow{} \Rspace$ two monotonic functions, and $F$ and $G$ be the respective sub-level set filtrations. For each dimension $d$, the bottleneck distance between the 
canonical harmonic diagrams $CHD(F)$ and $CHD(G)$ satisfies

\[ d_B(\chd(F), \chd(G)) \leq ||f-g||_\infty. \]

\end{theorem}


\subsection{Example}

We consider the same example we presented for instability, see Figure~\ref{fig:stableexample}. In the left complex, at time $t_4$ the first cycle is created and the cycle $z_1 = t_4+t_2-t_1$ is created and represents the top bar. At time $t_5$ the dimension of the harmonic chains increases, and one can see that the cycle $z_2 = t_2-t_1+t_3-t5$ is harmonic at $t_5$ and survives up to $t_9$. Among edges inserted until $t_5$, no cycle survives adding $t_8$ other than multiples of $z_2$. At $t_7$ are edges are present so therefore there has to be a cycle that survives until $t_{10}$. One checks that $z_3 = \partial(t_{10}) - 1/2 \partial (t_8 - t_9 )$ has this property.

At the right diagram, at time $t_4$ the cycle $z'_1 = -t_1+t_2+t_4-t_3$ is created and survives up to $t_9$. At time $t_5$, $z'_2 = t_5+t_4-t_3$ is created that survives up to $t_8$ and at time $t_7$ as before $z'_3=z_3$ is created and survives up to $t_{10}$.


\begin{figure}
    \centering
    \includegraphics{stableexample.eps}
    \caption{The canonical harmonic barcodes are stable.}
    \label{fig:stableexample}
\end{figure}

==> unused-sections/oldtext.tex <==


\subsection{The Orthogonal Harmonic Persistence Diagram}

We present a special harmonic persistence which is defined naturally from the filtration and therefore does not need the ordinary persistence barcode as an intermediary step. This is is significant since the bars define unique geometric features which do not depend on any choices made at all. This is of course true for any "natural" scheme of choosing basis elements for persistence barcode, however, the orthogonal harmonic persistence enjoys other favaroable properties too, see~\ref{}. 


Consider the filtration of the cycle groups obtained from the original filtration~\ref{eq:fcomplex}.

\begin{equation}\label{eq:fcycles}
    Z(K_0) \xrightarrow{f^H_0} Z(K_1) \xrightarrow{f^1} Z(K_2) \cdots \xrightarrow{f^{m-1}} Z(K_m).
\end{equation}

In the above, we denote the homomorphisms induced on the cycle groups also by $f_i$, $i=1,\ldots,m-1$. The coboundary homomorphism $\delta_n: C_n(K_i) \rightarrow C_{n+1}(K_i)$ is defined over all the chain group, and thus on the cycle group which is a vector sub-space. We thus have a homomorphism $\delta^Z_n : Z_n(K_i) \rightarrow C_{n+1}(K_i).$ Let $\har(K_i) \subset Z(K_i)$ be the kernel of $\delta^Z$ and let $Q(K_i)$ be the orthogonal complement of $\har(K_i)$ in $Z(K_i)$. We thus have $Z(K_i)/Q(K_i) \cong \har(K_i)$. We replace the $Z(K_i)$ in~\ref{eq:fcycles} by $Z(K_i)/Q(K_i)$. In general, for any complex $X$, let $Q(X)$ be the orthogonal complement of $\ker(\delta) \cap Z(X)$ in $Z(X)$.

The following proposition implies that there is a natural persistence module containing the spaces
$Z(K_i)/Q(K_i)$. This is an important fact which allows us to prove stability for this diagram.

\begin{proposition}\label{p:quotient}
Let $K$ and $L$ be simplicial complexes such that $K \subset L$. Let $f: Z(K) \rightarrow Z(L)$ be the homomorphism induced 
on the cycle groups by the inclusion. Then $f$ induces a quotient map $f^H: Z(K)/Q(K) \rightarrow Z(L)/Q(L)$. 
\end{proposition}




\begin{proof}
It is enough to prove the claim for the case when $L$ differs from $K$ by adding a simplex. The map $f$ then will be obtained as a composition.
We therefore assume that $L$ is obtained by adding the simplex $\sigma$ to $K$.

We recall that when a cochain $x$ satisfies $\delta(x)\neq 0$ in $K$, it satisfies $\delta(x) \neq 0$ in $L$, such that $K \subset L$. 
To prove that $f:Z_d(K) \rightarrow Z_d(L)$ induces a homomorphism on the quotient spaces, it is enough to prove that $f(Q_d(K)) \subset Q_d(L)$.
We consider three cases.

Case 1) $\dim(\sigma) < d$ or $\dim(\sigma) > d+1$. In this case, we have $Z_d(L) = Z_d(Q)$, and $\ker(\delta_{K,d}) = \ker(\delta_{L,d})$, therefore, $f$ is the identity homomorphism $Z(K)/Q(K) = Z(L)/Q(L)$.

Case 2) $\dim (\sigma) = d$. The difference from the previous case is that the cycle group $Z(L)$ might have gained one dimension. This happens if the simplex is positive, that is, if adding it creates a $d$-cycle $\nu \in Z_d(L)$. The harmonic cycles or $\ker^Z(\delta_{L,d})$ also gains one dimension and $\dim (Q_d(L)) = \dim (Q_d(K))$. 

Assume $z \in Q_d(K)$. Since the coboundary map is not changed, we have that $(z, (\ker\delta^Z_{L,d}f ))=0$. Therefore, $f(Q(K))$ is orthogonal to a co-dimension 1 subspace of $\ker(\delta^Z_{L,d})$. On the other hand, there is a cycle $y \in Z_d(L) -f(Z_d(K))$ which is orthogonal to $f(Z_d(K))= Z_d(K) \subset Z_d(L)$. We claim that $y$ is a cocycle. For any chain $c$, $\delta(y)(c) = y (\partial c) = (y, \partial c)=0$. The last inner product is zero since $\partial c$ is a chain in $Z_d(k)$, as the $d+1$ simplices are not changed from $K$. Therefore, $y$ is a cocycle. $f(Q_d(K))$ is also orthogonal to $y$ and therefore to all of $\ker(\delta^Z_{L,d})$. It follows that $Q_d(L) = f(Q_d(K))$.

Case 3) $\dim (\sigma) = d+1$. In this case the cycle space does not change, $Z(L) = Z(K)$, however, it might be that some $d$-cocycle is not a cocycle anymore.
%This decreases the dimension of $\ker(\delta_{i+1,d})$ resulting in an increase in dimension of $P(K_{i+1})$ and a reduce in dimension of the homology group which is isomorphic with $Z_d(K_{i+1})/P_d(K_{i+1})$. 
Since $\ker (\delta_{L,d}) \subset \ker(\delta_{K,d})$, for any $z \in Q(K)$, and any $\zeta \in \ker(\delta_{L,d})$, we have $(f(z), \zeta) = (z,\zeta) = 0$. Therefore, $f(Q(K)) \subset Q(L)$ which is what we wanted to prove.

\end{proof}


\begin{corollary}
The homomorphisms $f_i: Z(K_i) \rightarrow Z(K_{i+1})$ induce homomorphisms $f_i^H: Z(K_i)/Q(K_i) \rightarrow Z(K_{i+1})/Q(K_{i+1})$.
\end{corollary}

We thus obtain the following persistence module.

\begin{equation}\label{eq:fcycles}
    Z(K_0)/Q(K_0) \xrightarrow{f_0} Z(K_1)/Q(K_1) \xrightarrow{f_1} Z(K_2)/Q(K_2) \cdots \xrightarrow{f_{m-1}} Z(K_m)/Q(K_m).
\end{equation}

\paragraph{A more intuitive description}
Here we describe the orthogonal harmonic persistence by means of the ordinary persistence. Imagine sweeping the barcode from left to right. When we encounter a new bar, we simply take a basis element for homology that is orthogonal to the part of the homology group which already exists. This gives the scheme for choosing basis elements which we call \textit{the orthogonal scheme}. Note that as expected, this operation does not depend on any choices other than a constant multiplicative factor for the choice of harmonic cycle in homology with $\Rspace$ coefficients, such a choice does not affect the geometric shape of the cycle. 


\begin{proposition}
    The diagram obtained by the orthogonal scheme for choosing basis elements for persistent homology is equal to the orthogonal harmonic persistence diagram. 
\end{proposition}

The above description of orthogonal harmonic persistence also allows one to compute harmonic cycles
which represent the bars in the orthogonal harmonic barcode, see Section\ref{s:algorithms} for more detail.

\subsubsection{Example}
